Energy Sufficiency in Unknown Environments via Control Barrier Functions

Maintaining energy sufficiency of a battery-powered robot system is a essential for long-term missions. This capability should be flexible enough to deal with different types of environment and a wide range of missions, while constantly guaranteeing that the robot does not run out of energy. In this work we present a framework based on Control Barrier Functions (CBFs) that provides an energy sufficiency layer that can be applied on top of any path planner and provides guarantees on the robot's energy consumption during mission execution. In practice, we smooth the output of a generic path planner using double sigmoid functions and then use CBFs to ensure energy sufficiency along the smoothed path, for robots described by single integrator and unicycle kinematics. We present results using a physics-based robot simulator, as well as with real robots with a full localization and mapping stack to show the validity of our approach.

==> background.tex <==
\subsection{Control barrier functions}
A control barrier function is a tool that has gained much attention lately as a way of enforcing set forward invariance to achieve safety in control affine systems of the form 
\begin{equation*}
\dot{\mathbf{x}} = f(\mathbf{x})+g(\mathbf{x})u
\end{equation*}
where $u\in U\subset \mathbb{R}^m$ is the input, $U$ is the set of admissible control inputs, and $\mathbf{x}\in\mathbb{R}^n$ is the state of the system, and here $f$ and $g$ are both Lipschitz continuous. In this context, what is meant by safety is achieving set forward invariance of some safe set $\mathcal{C}$, meaning that if the states start in $\mathcal{C}$ at $t=t_0$, they stay within $\mathcal{C}$ for all $t>t_0$. This safe set $\mathcal{C}$ is defined as  the superlevel set of a continuously differentiable function $h(x)$ in the following manner \cite{ames2019control}:

\begin{equation}
\begin{split}
\mathcal{C} &= \{x\in\mathbb{R}^n:h(x)\geq 0\}\\
\partial\mathcal{C} &= \{x\in\mathbb{R}^n:h(x)=0\}\\
Int(\mathcal{C}) &= \{x\in\mathbb{R}^n:h(x)>0\}
\end{split}
\end{equation}
This can be achieved by finding a value of control input that satisfies $\dot{h}\geq -\alpha(h)$, with $\alpha(h)$ being an extended class $\mathcal{K}$ function \cite{khalil2002nonlinear}.

\begin{definition}{\cite{ames2019control}}
	For a subset $\mathcal{W}\subset \mathcal{C}$, a continuously differentiable function $h(x)$ is said to be a zeroing control barrier function (ZCBF) if there exists a function $\alpha(h)$ s.t. 
	\begin{equation}
	\sup_{u\in U}L_fh+L_ghu\geq -\alpha(h), \quad \forall x\in \mathcal{W}
	\end{equation} 
	where $L_fh$ and $L_gh$ are the Lie derivatives of $h(x)$ in direction of $f$ and $g$ respectively.
\end{definition}

Supposing that we define the set of all safe inputs 
$U_{s} = \{u\in U: L_fh+L_ghu\geq -\alpha(h)\}$, then any Lipschitz continuous controller $u\in U_s$ guarantees that $\mathcal{C}$ is forward invariant \cite{ames2019control}.
Since the nominal control input $u_{nom}\in U$ for a mission may not belong to $U_s$, there should be a way to enforce safety over the nominal mission input. This could be done by the following quadratic program (QP)~\cite{ames2019control}

\begin{equation}
\begin{aligned}
&  u^*=\underset{u}{\text{min}}
& & ||u-u_{nom}||^2 \\
& \quad \quad \quad \text{s.t.}
& & L_fh(x)+L_ghu \geq -\alpha(h) \\
%&&& X \succeq 0.
\end{aligned}
\label{eqn:QP}
\end{equation}
noting that $u^*$ tries to minimize the difference from $u_nom$, as long as safety constraints are not violated.

\subsection{Bezier curves}

In this work we use 2D Bezier curves to describe paths along which we want the robot to move. A Bezier curve describes a parametric relationship between $(x,y)$ pairs and a parameter $\tau\in[0,1]$ which describes the progression along the curve, i.e. $\tau = 0$ means the beginning of the curve and $\tau=1$ is its end. A Bezier curve of order $n$ is defined by a set of $n+1$ control points $P_c\in\mathbb{R}^{(n+1)\times 2}$ (i.e. each column corresponds to one coordinate), and a point along the curve is defined in the following manner:

\begin{equation}
p(\tau) = \sum_{i=0}^{n}P_{c_i}B_{i}^{n}(\tau)
\end{equation}
where $B_{i}^{n}(\tau)$ are Bernstein polynomials. An equivalent matrix representation is
\begin{equation}
p(\tau) = T^T(\tau) B P_c
\label{eqn:bezier_point}
\end{equation}
where $p(\tau)\in\mathbb{R}^{1\times 2}$,$T(\tau)\in\mathbb{R}^{n+1}$ and defined as 
\begin{equation}
T(\tau) = \begin{bmatrix}
1&\tau&\tau^2\dots\tau^{n}
\end{bmatrix}^T
\label{eqn:T}
\end{equation}
and $B$ is a matrix containing coefficients of Bernstein polynomial, and is expressed as $B = DN$ where $N_{ij} = \binom{i}{j}(-1)^{j-1}$ for $ i=0,\dots,n$ and $j=0,\dots,i$, and $D$ is a diagonal matrix whose elements are $D_{jj} = \binom{n}{j}(-1)^{j-1},\quad j = 0,\dots,n$. 

The derivative of the Bezier curve wrt $\tau$ is expressed as
\begin{equation}
p^\prime(\tau) = T^{\prime^T}BP_c
\label{eqn:bez_derivative}
\end{equation}
where 
\begin{equation}
T^\prime(\tau) = \begin{bmatrix}
0&1&2&6\tau\dots n\tau^{n-1}
\end{bmatrix}^T
\label{eqn:t_prime}
\end{equation}
and higher derivatives can be obtained in a similar manner as well. 

The arc length of a Bezier curve from a point $p(s)$ on the curve (where $s\in[0,1]$ is a progression parameter) to the end of the curve (where $s=1$) is expressed as
\begin{equation}
L = \int_{s}^{1}\sqrt{\tfrac{dp_x}{d\tau}^2+\tfrac{dp_y}{d\tau}^2}d\tau
\label{eqn:len_bez}
\end{equation}
with $p(\tau)=\begin{bmatrix}
p_x&p_y
\end{bmatrix}^T$.
Although there is no closed form solution for calculating the length of a general Bezier curve, it can be approximated with a high degree of accuracy using numerical integration with Gaussian quadratures, so the length can be approximated with the $m^{th}$ degree polynomial as
\begin{equation}
L = \int_{-1}^{1}f(\tau)d\tau \approx \sum_{i=1}^{m}c_if(\tau_i)
\end{equation}
where $f(\tau) = \sqrt{\tfrac{dp_x}{d\tau}^2+\tfrac{dp_y}{d\tau}^2}$. One issue with this form is that $\tau\in[0,1]$, so to calculate the length of a segment starting at $\tau = s$ and ending at $\tau = 1$, the integration limit and integrand are modified to be 
\begin{equation}
L = \tfrac{1-s}{2}\int_{s}^{1}f(\tfrac{1-s}{2}\tau+\tfrac{1+s}{2})d\tau\approx \tfrac{1-s}{2}\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})
\label{eqn:bez_len}
\end{equation}
%\todo{mention something about the error of the estimation using the gauss quadrature}
%The approximation error due to the Gauss quadrature integration is 
\subsection{Approximate merging of Bezier curves\label{sec:merging}}
One useful idea that we use  in our framework is the ability to construct a larger Bezier curve from smaller Bezier curve segments. Generally speaking, there is no analytical solution for merging general order Bezier curves \todo{add a reference for this claim}. In this work we adopt the method presented in \cite{lu2015explicit} which provides an explicit expression for the control points of a Bezier curve that approximates a set of connected Bezier curve segments.

Suppose there are $K$ Beizer segments, each segment with control points $P^k$. The main goal is to find a set of control points $R_n$ for a Bezier curve of order $n$ that minimizes the $L_2$ distance between the original segments and the approximate merging curve, expressed as
\begin{equation}
E = \sum_{k = 1}^{K}\Delta \tau_k \int_{1}^{1}||B_nS_kR_{n} - B_{n_k}P_{n_k}^{k}||^2d\tau
\end{equation}
where $B_n$ is expressed as $B_n=T^TB$ (from equation \eqref{eqn:bezier_point}), $S_k = D_2(\tfrac{\tau_k}{\tau_{k+1}})D_1(\tau_{k+1})$ where
\begin{equation*}
D_1(\lambda) = \begin{bmatrix}
1&0&\dots&0\\B_{0}^1(\lambda)&B_{1}^1(\lambda)&\dots&0\\\vdots&\vdots&\ddots&\vdots\\B_{0}^n(\lambda)&B_{0}^1(\lambda)&\dots&B_{n}^n(\lambda)
\end{bmatrix}
\end{equation*}
and
\begin{equation*}
D_2(\lambda) = 
\begin{bmatrix}
B_{0}^n(\lambda) & B_{1}^n(\lambda)&\dots&B_{n}^n(\lambda)\\0&B_{0}^{n-1}(\lambda)
&\dots&B_{0}^{n-1}(\lambda)\\
\vdots&\vdots&\ddots&\vdots\\
0&0&\dots&1
\end{bmatrix}
\end{equation*}
We note that $S_kR_n$ represents the control points of merging curve subdivision (of order $n$) on interval $[\tau_k,\tau_{k+1}]$ corresponding to the original segment $k$ (of order $n_k$) with control points $P^{k}_{n_k}$.

The merging curve satisfies the following $C^{d_1}$ and $C^{d_2}$ continuity conditions at both ends
\begin{equation}
\begin{split}
\frac{d^i r(0)}{d\tau^i} &= \frac{d^i p^1(0)}{d\tau^i}, \quad i = 0,\dots,d_1\\
\frac{d^i r(1)}{d\tau^i} &= \frac{d^i p^K(1)}{d\tau^i}, \quad i = 0,\dots,d_2
\end{split}
\label{eqn:ends_cont}
\end{equation}
The main idea is to divide the control points $R_n$ to two sets of points: constrained points $R_n^c = R_n(I_n^c)$ and free points $R_n^f= R_n(I_n^f)$, with $I_n^c \coloneqq\{0,\dots,d_1,n-d_2,\dots,n\}$ and $I_n^f\coloneqq\{d_1+1,\dots,n-d_2-1\}$ being the indices of constrained and free control points respectively.
The constrained control points are calculated uniquely to satisfy \eqref{eqn:ends_cont} \cite{farin2002curves} and we state the results for the sake of completeness. We can represent $R_n^c$ as  
\begin{equation}
R_n^c = \begin{bmatrix}
R_{c_1}\\R_{c_2}
\end{bmatrix}
\end{equation}
where
\begin{equation}
\begin{split}
R_{c_1} &= \overbrace{\Gamma_1^{-1}\begin{bmatrix}
1&0&0\\0&\tfrac{d_1}{n}&0\\0&0&\tfrac{d_1(d_1-1)}{n(n-1)}
\end{bmatrix}\Gamma_1}^{\Phi_1}\begin{bmatrix}
P_1^0\\P^1_1\\P^1_2
\end{bmatrix}\\
R_{c_2}&=\underbrace{\Gamma_2^{-1}\begin{bmatrix}
\tfrac{d_2(d_2-1)}{n(n-1)}&0&0\\0&\tfrac{d_2}{n}&0\\0&0&1
\end{bmatrix}\Gamma_2}_{\Phi_2}\begin{bmatrix}
P^{K}_{n_K-2}\\P^{K}_{n_K-1}\\P^{K}_{n_K}
\end{bmatrix}
\end{split}
\label{eqn:Rc}
\end{equation}
with $\Gamma_1$ and $\Gamma_2$ defined as 
\begin{equation}
\Gamma_1=\begin{bmatrix}
1&0&0\\-1&1&0\\1&-2&1
\end{bmatrix},\Gamma_2 = \begin{bmatrix}
1&-2&1\\0&-1&1\\0&0&1
\end{bmatrix} 
\end{equation}
The free points can then be calculated as follows
\begin{equation}
R_n^f = H_{ff}^{-1}\left(-H_{fc}R_n^c+\sum_{K}^{k=1}\Delta\tau_k (S_k^f)^TG_{n,n_k}P_{n_k}^k\right)
\label{eqn:Rf}
\end{equation}
where $S_k^c \coloneqq S_k(\dots;I_n^c)$, $S_k^f \coloneqq S_k(\dots;I_n^f)$ (meaning taking columns of $S_k$ corresponding to indices $I_n^c$ and $I_n^f$ respectively), $H_{fc}$ and $H_{ff}$ are defined as 
\begin{equation}
\begin{split}
H_{fc} &= \sum_{K}^{k=1}\Delta\tau_k (S_k^f)^TG_{n,n}S_k^c
\\
H_{ff} &= \sum_{K}^{k=1}\Delta\tau_k (S_k^f)^TG_{n,n}S_k^f
\end{split}
\end{equation}
Where $G_{n,m}$ is a $(n+1,m+1)$ matrix with elements defined as 
\begin{equation}
g_{i,j} = \frac{1}{n+m+1}\frac{\binom{n}{i}\binom{m}{j}}{\binom{n+m}{i+j}}
\end{equation}
for $i=0,\dots,n$ and $ j = 0,\dots,m$. The total set of control points for the merged Bezier curve is
%\begin{equation*}
%R_n = \begin{bmatrix}
%R_{c_1}\\R_n^f\\R_{c_2}
%\end{bmatrix}
%\end{equation*}
\begin{equation}
R_n = \begin{bmatrix}
R_{c_1}^T&(R_n^f)^T&R_{c_2}^T
\end{bmatrix}^T
\label{eqn:Rn}
\end{equation}

\subsection{Problem definition} 
We adopt simple single integrator dynamics to describe the robot position, as well as a simple exponential discharge model for voltage change
\begin{equation}
\begin{split}
\dot{x} &= u\\
\dot{V} &= -k_d V
\end{split}
\label{eqn:robot_dynamics}
\end{equation}
with $x\in\mathbb{R}^2$ being the robot's position , $u\in\mathcal{U}\in\mathbb{R}^2$is the control action, $V > 0$ is the battery voltage and $k_d > 0$ is a conservative estimate of discharge rate. 
Suppose that there exists a path between the robot and the charging station which is described by a set of waypoints $\mathcal{W}=\begin{bmatrix}
w_0^T&w_1^T&\dots&w_{n_w-1}^T
\end{bmatrix}^T$, with $w_i\in\mathbb{R}^{2}$ and the charging station is at $w_{n_w-1}$, produced by a path planner every $\mathcal{T}$ seconds. Provided that such robot is carrying out a mission encoded by a nominal control action $u_{nom}$, our objective is to ensure energy sufficiency for this robot, i.e. robot's voltage is always above a certain desired threshold $V_{min}$, while taking the path defined by $\mathcal{W}$ back to the charging station. Such scenario is relevant in cases where ground robots are doing missions in cluttered environments or flying robots in areas with no fly zones.

In this work we adopt the following assumptions:
\begin{enumerate*}
	\item The communication graph between the robots is a complete graph. 
	\item The battery discharge rate is uniform over the environment.
	\item The paths produced by the path planner are two-way traversable.
\end{enumerate*}

==> coordination.tex <==
Provided that a robot has a method to ensure energy sufficiency as discussed in previous sections, multiple robots can then coordinate temporally the use of a common charging station. In this section we adapt our coordination framework proposed in \cite{fouad2022energy}. The main idea is to calculate the arrival time of each robot to the charging station based on a conservative estimate of its voltage discharge, and then change the values of $V_{m}$ in \eqref{eqn:energy_suff_cbf} so that the differences between robot's arrival times are adequately separated. We follow \cite{fouad2022energy} by using the following dynamics for the value of $V_{m}$ in \eqref{eqn:energy_suff_cbf}
\begin{equation}
\dot{V}_{m} = \mu
\end{equation}
for a control input $\mu\in\Theta=\mathbb{R}$, with $\Theta$ being the set of admissible values of $\mu$. As a result the constraint \eqref{eqn:suff_constraint} will be modified to be
\begin{equation}
-k_eV-\frac{k_e}{v_r}(V-h_e)\frac{dL}{dt}-\mu e^{\tfrac{k_e}{v_r}(L(s)-\delta)} \geq -\gamma_e h_e
\label{eqn:suff_cond_mod}
\end{equation}
%We start by describing some tracking properties of \eqref{eqn:energy_suff_cbf} that will help estimating arrival times.

%\begin{lemma}
%	For a robot with dynamics as in \eqref{eqn:robot_dynamics} and applying the constraint associated with the ZCBF defined in \eqref{eqn:energy_suff_cbf}, then $V-V_{m}$ is bounded by a quantity that decays exponentially with $\gamma_e$.
%\end{lemma}
%\begin{proof}
%	To show this, we point out that using a control action $\eta$ and $\mu$ that satisfy \eqref{eqn:suff_cond_mod} then $h_e$ will decay exponentially as demonstrated in lemma \ref{lemma:2}. Supposing that $L(s) = \delta$ at some time $t_a$, then from \eqref{eqn:exp_decay}
%	\begin{equation}
%	V-V_{m} = h_{e_0}e^{-\gamma_e(t-t_0)}
%	\end{equation}
%	which means that such difference can be arbitrarily small by choosing higher value of $\gamma_e$, and is bounded from below by zero by virtue of $h_e$ being a ZCBF.
%\end{proof}

By virtue of \ref{lemma:base} $V=V_m$ at $L(s)=\delta$ for the reference point $x_r$, and given that we are using a constant conservative estimate of discharge rate $k_e$, the time of arrival can be estimated as the time needed to reach $V=V_{m}$ from a voltage $V$. The arrival time $T_a$ and its derivative can be expressed as
% \todo{check the effect of $\epsilon$ on arrival time}
\begin{equation}
\begin{split}
T_a &= \tfrac{1}{k_e}\log\tfrac{V}{V_{m}}\\
\Rightarrow\dot{T}_{a} &= -1 - \tfrac{\mu}{ke V_{m}}
\end{split}
\label{eqn:arrival_time}
\end{equation}

As discussed earlier, the energy sufficiency framework described so far leads the robot to enter the charging region such that $V\nless V_m$ at $||x-x_c|| = \delta$ , and if $V=V_m$ at $L(s) = \delta$ (inside the charging region), this means that the robot arrives on the boundary earlier than the time it takes to get to $V=V_m$. We attempt to study the effect of such phenomenon on the arrival time.

\begin{lemma}
	\label{lemma:time_slack}
	For a robot carrying out the control strategy in \eqref{eqn:QP_suff} and supposing the free end assumption \eqref{eqn:term_cond} for the Bezier path interpolation was adopted at the charging station location, as well as having the nearest waypoint to the charging station outside of the charging region, i.e. $||x_c - w_{n_w-2}|| > \delta$, then there will be no inflection in the Bezier segment between $w_{n_w-2}$ and $w_{n_w-1}$ (between the charging region center and the first waypoint). Moreover, the length of the Bezier curve segment inside the charging region is less than $2\delta$.
\end{lemma}

\begin{proof}
	Considering the third order Bezier segment $p(\tau)$ between $w_{n_w-2}$ and $w_{n_w-1}$, i.e. the center of the charging region and the first waypoint, according to \eqref{eqn:t_prime} then the second derivative of the path is 
	\begin{equation}
	p^{\prime\prime}(\tau) = 6\left[(1-\tau)P_0 + (-1+\tau)P_1 + (1-3\tau)P_2 + \tau P_3\right]
	\label{eqn:sec_der}
	\end{equation}
	where $P_i$ are the segment's control point, $P_0 = w_{n_w-2}$ and $P_3 = w_{n_w-1}$. At $\tau = 1$, \eqref{eqn:sec_der} will be equal to zero so
	\begin{equation}
	P_1 - 2P_2 + P_3 = 0
	\label{eqn:free_end}
	\end{equation}
	substitute \eqref{eqn:free_end} in \eqref{eqn:sec_der} we have
	\begin{equation}
	p^{\prime\prime}(\tau) = 6(1-\tau)(P_0-P_1+P_2)
	\label{eqn:free_end_2}
	\end{equation}
	and since $(P_0-P_1+P_2)$ does not change in $\tau$ (as $P_i$ are control points), then \eqref{eqn:free_end_2} does not change signs on this segment and no inflection takes place.
	\begin{figure}[!htb]
		\centering
		\fontsize{15pt}{15pt}\selectfont% or whatever fontsize you like
		\def\svgwidth{5.333in}
		\scalebox{0.3}{\input{charging_region2.pdf_tex}}
		\caption{General case of a  portion of the last Bezier segment entering the charging region with free end interpolation condition at $x_c$. The blue curve shows the range of extension that the curved segment $A-x_c$ can undergo while being in circle.
%		The red segment is the portion of path between arriving at the boundary of charging region (point $A$) and the point at which $L(s) = \delta$ and $V=V_m$ (point $x^\prime$).
		}
		\label{fig:charging_region2}
	\end{figure}
	We note that when the reference point $x_r$ arrives to the boundary where $V > V_m$ there will be a certain amount of time $\Delta_t$ till it reaches $x^\prime$ where $V = V_m$ and $L(s) = \delta$, which is the difference between the actual arrival time and estimated one from \eqref{eqn:arrival_time}. Such estimate could be the difference in distance $\epsilon^\prime$ (red segment in figure \ref{fig:charging_region2}) divided by $v_r$ (since the reference point moves along the path with a speed equal to $v_r$ as shown in lemma \ref{lemma:2}). Consider the Bezier segment inside the charging region, then it can be inscribed in an equilateral triangle of side length $\delta$, shown in figure \ref{fig:charging_region2}, which demonstrates that pathologically this segment can't be of length greater than $2\delta$ to be inside the circle (demonstrated by the blue curve). Moreover, at such extreme curve inflection will takes place which violates \eqref{eqn:free_end_2}. Therefore \begin{equation}
	\delta + \epsilon^\prime < 2\delta \Rightarrow \epsilon^\prime < \delta \Rightarrow \Delta_t =\tfrac{\epsilon^\prime}{v_r}<\tfrac{\delta}{v_r}
	\label{eqn:slack_time}
	\end{equation}.
\end{proof}


The last lemma gives a conservative estimate of how much earlier the robot's reference point arrives to the station's boundary compared to when it expects to arrive according to \eqref{eqn:arrival_time}. 
\begin{remark}\todo{is this a good remark?}
	We note that from a practical point of view, using a high value  of $\beta_2$ in \eqref{eqn:cont_cond} leads to having a Bezier path that closely follows the piecewise linear path from the path planner, thus the reference point $x_r$ reaches the boundary at almost $V=V_m$ and the effects addressed in lemma \ref{lemma:time_slack} and proposition \ref{proposition:length_error} become less pronounced.
\end{remark}
We use the same coordination framework in \cite{fouad2022energy} with the time of arrival described in \eqref{eqn:arrival_time}, but we include the general framework for the sake of completeness. We assume a complete graph communication between robots \cite{fouad2022energy}. We summarize the coordination framework in the following points:
\begin{itemize}
	\item Defining a candidate CBF $h_{c_{ij}}$ with an associated pairwise coordination safe set $\mathcal{C}_{ij}$, the purpose of which is to adjust $V_m$ values to make a pair of agents avoid each other's arrival time.
	\item A candidate CBF $h_{L}$ that bounds the value of $V_m$ from below to prevent the robot from reaching the charging station with a voltage less than a hard lower bound $V_{lb} > 0$ related to battery characteristics (otherwise the value of $V_m$ can keep decreasing to satisfy $h_e>0$ without moving the robot back to the station).
	\item A compositional CBF consisting of all previous CBFs to ensure the feasibility of the final QP in \eqref{eqn:QP}.
\end{itemize}. We define the pairwise coordination safe set $\mathcal{C}_{ij}$ between two robots $i$ and $j$ as
\begin{equation}
\mathcal{C}_{ij} = \{(V_{m_i},V_{m_j})\mathbb{R}^2: h_{c_{ij}}\geq 0, \forall j\in\mathcal{N}^\prime_i\}
\end{equation}
where $\mathcal{N}^\prime_i$ is the set of neighbours of agent $i$ and $h_{c_{ij}}$ is a candidate CBF defined as 
\begin{equation}
h_{c_{ij}} = \log\tfrac{|T_{a_i}-T_{a_j}|}{\delta_T}
\end{equation}
where $\delta_T = \delta_t + \Delta_t > 0$, $\delta_t$ is the desired separation in arrival times between two robots, and $\Delta_t$ is defined in \eqref{eqn:slack_time}. The constraint associated with $h_{c_{ij}}$ is 
\begin{equation}
\tfrac{T_{a_i}-T_{a_j}}{|T_{a_i}-T_{a_j}|^2}(\dot{T}_{a_i}-\dot{T}_{a_j})\geq -\gamma_c h_{c_{ij}}
\label{eqn:hc_constraint}
\end{equation}
and since agent $i$ has access only to $\mu_i$ the last inequality becomes
\begin{equation}
-\tfrac{T_{a_i}-T_{a_j}}{|T_{a_i}-T_{a_j}|^2}\tfrac{\mu_i}{V_{m_i}}\geq -\gamma_ch_{c_{ij}}
\label{eqn:hc_constraint_2}
\end{equation}
The CBF candidate for bounding $V_m$ from below is 
\begin{equation}
%h_{L_{i}} = k_p(V_{m_i}-V_{lb})
h_{L_{i}} = k_p
\log \tfrac{V_{m_i}}{V_{lb}}
\end{equation}
for $k_p>0$ is a scaling gain. The constraint associated with $h_{L_{i}}$ is
\begin{equation}
%k_p\mu_i \geq -\gamma_L h_{L_i}
k_p\tfrac{\mu_i}{V_{m_i}} \geq -\gamma_L h_{L_i}
\label{eqn:lower_bound_const}
\end{equation}
It can be shown that both $h_{c_{ij}}$is indeed a ZCBF.
\begin{lemma}{\cite{fouad2022energy}}\todo{talk about converging to $\delta_T$ makes you safe for $\delta_t$}
	For a pair of robots described by \eqref{eqn:robot_dynamics} and applying \eqref{eqn:hc_constraint_2} as a constraint in the QP \eqref{eqn:QP}, $h_{c_{ij}}$ is a ZCBF provided that $T_{a_i}(t_0)\neq T_{a_j}(t_0)$ and $\mu_i\in\Theta=\mathbb{R}$.
\end{lemma}
Also $h_{L_i}$ can be shown to be a ZCBF, since $\mu_i\in\Theta=\mathbb{R}$ then there is always a value of $\mu_i$ that satisfies the inequality \eqref{eqn:lower_bound_const}. These pairwise coordination constraints can be potentially contradicting, and they can contradict the lower bound constraint \eqref{eqn:lower_bound_const} (due to the fact that several constraint attempt to affect a one dimensional variable $V_m$ that is changing along a line~\cite{fouad2022energy}). We use a boolean nonsmooth CBF \cite{glotfelter2018boolean} to compose the final coordination CBF \cite{fouad2022energy} and it takes the form
\begin{equation}
h_{c_i} = \bigwedge\limits_{j\in\mathcal{N}_{i}^{\prime}}h_{c_{ij}}\wedge h_{L_i}
\end{equation}
where $\wedge$ signifies an AND operator.
\begin{remark}
	In this work, as in \cite{fouad2022energy}, we assume the that a robot arrives to the charging station and spends a certain amount of time $T_{ch}$ doing a recharge using battery swapping. This implies the existence of a maximum limit on the desired temporal separation between arrivals and this limits depends on the number of robots in the charging cycle, discharge rate $k_e$ and the lower bound of voltage on arrival $V_{lb}$ as demonstrated in \cite{fouad2022energy}.
\end{remark}
\begin{remark}
	We introduce a discrete state jump $V_m = V_{lb}$ when a robot arrives to the charging station to achieve maximal utilization in arrival time separation as we demonstrate in \cite{fouad2022energy}, where it is shown that such change in the value of $V_m$ does not violate the coordination safety as introduced above.
\end{remark}

==> dynamic1.tex <==
We extend the results from the previous section to a scenario in which the robot is at an arbitrary position that is not necessarily at the starting point of the Bezier path (i.e. $h_d<0$ at $s=0$). We solve this problem by creating a new Bezier curve that includes the robot's position as its beginning control point at $s=0$ for the new curve. We create an extension curve from the current position to the head of curve, then we create a new approximate Bezier curve that merges the original path and its extension, and finally we apply the same result from the previous section to let the robot move along the extended Bezier path back to the charging station.

%The main idea is to create a new Bezier curve that joins the position of the robot to the beginning of the original Bezier path, then we create a new Bezier curve of higher order that approximate these two Bezier curves together (the original curve and the additional extension). We then apply the same idea from the previous section to let the robot move along the new higher order Bezier path back to the charging station.



\subsection{Bezier extension}

We first create a continuous Bezier segment of order $l$, we call it $q(\tau)$ and specified with control points $Q_c\in\mathbb{R}^{(l+1)\times 2}$, from a point $x_f\in\mathbb{R}^2$ (that follows the robot's current position in a manner that will be described in the next section) to the head of the original Bezier curve which will be the junction point. We impose $G^1$ continuity conditions at the junction between the two segments. This implies continuity at the junction point and continuity of derivative vector direction and these conditions are expressed as  
\begin{equation}
\begin{split}
&q(1) = p(0)\\
&\tfrac{\partial q}{\partial \tau}(1) = \zeta \tfrac{\partial p}{\partial \tau}(0), \quad \zeta > 0
\end{split}
\label{eqn:continuity}
\end{equation}
For the sake of simplicity we choose $l = 2$ since this is the least order needed for the Bezier extension to have a non zero derivative, i.e. to be able to impose $G^1$ continuity condition. We consider $q(0)=x_f$, and the goal is to calculate the other two control points so that conditions in \eqref{eqn:continuity} are satisfied. The conditions \eqref{eqn:continuity} can be alternatively expressed as 
\begin{equation}
\begin{split}
&\hat{T}_{q}(1)\hat{B}_q\hat{Q}_c = T_{p}(0)B_pP_c\\
&\hat{T}_{q}^{\prime}(1)\hat{B}_q\hat{Q}_c = \zeta T_{p}^{\prime}(0)B_pP_c
\end{split}
\label{eqn:q_con}
\end{equation}
where $\hat{Q}_c\in\mathbb{R}^{l\times 2}$ is such that $Q_c = \begin{bmatrix}
x_f^T&\hat{Q}_c^T
\end{bmatrix}^T$ and $\hat{B}_q$ is a $l\times l$ matrix comprised of the last $l$ rows and $l$ columns of a $l^{th}$ order Bernstein polynomial coefficients matrix . $\hat{T}_q(\tau)$ and $\hat{T}_q^\prime(\tau)$ are the last $l$ elements of $T(\tau)$ and $T^\prime(\tau)$ as defined in \eqref{eqn:T} and \eqref{eqn:t_prime} respectively. We can express \eqref{eqn:q_con} in a matrix form 
\begin{equation*}
\underbrace{\begin{bmatrix}
\hat{T}_{q}(1)\\\hat{T}_{q}^\prime(1)
\end{bmatrix}\hat{B}_q}_{\lambda_q} \hat{Q}_c = \underbrace{\begin{bmatrix}
T_p(0)\\\zeta T_p^\prime(0)
\end{bmatrix} B_p}_{\lambda_p} P_c
\end{equation*}
and the value of $\hat{Q}_c$ can be calculated as
\begin{equation}
\hat{Q}_c = (\lambda_q^T\lambda_q)^{-1}\lambda_q^T\lambda_pP_c
\end{equation}
We note that $\zeta$ in the above equations act as a shape parameter that controls the flatness of the Bezier extension. Figure shows the effect of changing $\zeta$ for a given Bezier curve. We use the approximate merging method described in section \ref{sec:merging} to find a higher order Bezier curve that merges the original Bezier curve (with control points $P_c$) and the extension (with control points $Q_c = \begin{bmatrix}x_f^T&\hat{Q}_c^T
\end{bmatrix}^T$) and the control points of the new $n^{th}$ order Bezier curve are  
\begin{equation}
\mathcal{Q}=\begin{bmatrix}
x_f &\mathcal{Q}^{C^T} &P_{c_N}^T
\end{bmatrix}^T
\label{eqn:Q}
\end{equation}
where $\mathcal{Q}^C$ is as defined in \eqref{eqn:merge} (with $Q_0 = x_f^T$ and $P_N = P_{c_N}$), and $P_{c_N}$ is the last control point of the original Bezier path $p(\tau)$. 

\subsection{Energy sufficiency over merging Bezier curve}
We can now extend the method outlined in section \ref{sec:static} to be applicable on the approximate Bezier curve that merges the original path and its extension. We modify \eqref{eqn:dL} to account for the temporal change in control points of the merging Bezier curve due to the robot's motion
\begin{equation}
\begin{split}
\frac{dL}{dt} &= \frac{\partial L}{\partial s}\frac{ds}{dt}+\frac{\partial L}{\partial t}= \frac{\eta}{2}\left[-\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right.\\&\left.+(1-s)\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right]+
\\&\frac{1-s}{2}\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial t}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})
\end{split}
\label{eqn:dL2}
\end{equation}
where $f(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = ||A_i||$, $\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})=\tfrac{1}{||A||}AA^{\prime^T}$, $\tfrac{\partial f}{\partial t}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})=\tfrac{1}{||A||}A\dot{A}^T$, and  
\begin{equation}
\begin{split}
A_i &= T^{\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})B\mathcal{Q}\\
A_{i}^{\prime} &=\tfrac{1-\tau_i}{2} T^{\prime\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})B\mathcal{Q}\\
\dot{A}_i &= T^{\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})B\tfrac{\partial\mathcal{Q}}{\partial t}
\end{split}
\label{eqn:A2}
\end{equation}
finally $\tfrac{\partial\mathcal{Q}}{\partial t}$ is expressed as 
\begin{equation}
\tfrac{\partial\mathcal{Q}}{\partial t} = \begin{bmatrix}
\dot{x}_f &\dot{\mathcal{Q}}^{C^T}& 0_{1\times 2}
\end{bmatrix}^T
\end{equation}
with $\dot{\mathcal{Q}}=-\left(\mathcal{A}^{C^T}\mathcal{A}^{C}\right)^{-1}\mathcal{A}^{C^T}\dot{x}_f^T$

%The Bezier extension we discussed previously is created such that it extends the original Bezier curve to a point $x_f$ that follows the robot's position. The reason that we use $x_f$ instead of robot's actual position is that fact that the merging path will keep changing when the robot goes back to the charging station, which is problematic because the method developed for following Bezier paths in the previous section requires having a fixed Bezier path along which the robot moves back to the charging station. 

We note that there is a singularity in the system when 

The value of $x_f$ in previous relations change according to the following relation

%Therefore we need to change $x_f$ so that it closely follows the robot as long as it does not need to return back to the charging station, but stops as soon as the robot starts heading back. To do this we use the following control law
\begin{equation}
\dot{x}_f = -k_p(x_f-x)\xi(s)=-k_p(x_f-x)\left(1-\tfrac{1}{1+e^{-\beta(s-\upsilon)}}\right)
\label{eqn:track}
\end{equation}
where $\beta\gg 0$ and $0<\upsilon\ll1$. We explain the reason for this choice in the next lemma
\begin{lemma}
	For a robot with dynamics described in \eqref{eqn:robot_dynamics} that uses the candidate CBF in \eqref{eqn:energy_suff_cbf} to follow an approximate Bezier path defined by points \eqref{eqn:Q}, and using the constraint in \eqref{eqn:suff_constraint} with $\tfrac{dL}{dt}$ defined in \eqref{eqn:dL2} and $x_f$ that changes according to \eqref{eqn:track}, then \eqref{eqn:energy_suff_cbf} is a ZCBF.
\end{lemma}

%The idea behind \eqref{eqn:track} is that $x_f$ follows the robots current position, but as soon as $s$ starts increasing (indicating that the reference point $x_r$ starts moving along the Bezier path towards the charging station), then the value of $\xi(s)$ will rapidly go to zero which will freeze the value of $x_f$.

==> dynamic2.tex <==
We extend the results from the previous section to consider the case in which the control points of the Bezier path are changing with time due to robot's movement and discrete changes in path due to path planner input. 
\subsection{Effect of robot's movement}
Supposing that the waypoint list is constant, the main difference from the static case is the fact that the path's control points $R_n$ are changing due to the change in robot's position. As a result \eqref{eqn:dL} will become
\begin{equation}
\begin{split}
\frac{dL}{dt} &= \frac{\partial L}{\partial s}\frac{ds}{dt}+\frac{\partial L}{\partial t}= \frac{\eta}{2}\left[-\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right.\\&\left.+(1-s)\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right]\\&+\tfrac{1-s}{2}\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial t}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})
\end{split}
\label{eqn:dL2}
\end{equation}
to express $\tfrac{\partial f}{\partial t}$ we define $A_{t_i}\in\mathbb{R}^{1\times2}$ as
\begin{equation}
\begin{split}
A_{t_i} &= T^{\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})B\frac{\partial R_n}{\partial t}
\end{split}
\label{eqn:At}
\end{equation}
and $\tfrac{\partial f}{\partial t}$ then is expressed as 
\begin{equation}
\frac{\partial f}{\partial t}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = \tfrac{1}{||A_i||}A_iA_{t_i}
\label{eqn:pf_pt}
\end{equation}
where $A_i$ is as defined in \eqref{eqn:A} and $\tfrac{\partial R}{\partial t}$ is 
\begin{equation}
\frac{\partial R_n}{\partial t} = \begin{bmatrix}
\frac{\partial R_{c_1} }{\partial t}^T&\frac{\partial R_n^f }{\partial t}^T&\frac{\partial R_{c_2} }{\partial t}^T
\end{bmatrix}^T
\end{equation}
where 
\begin{equation}
\tfrac{\partial R_{c_1}}{\partial t} = \Phi_1\begin{bmatrix}
\partial \bar{w}_0/\partial t\\\partial a_0/\partial t\\\partial b_0/\partial t
\end{bmatrix}, 
\tfrac{\partial R_{c_2}}{\partial t} = \Phi_2\begin{bmatrix}
\partial b_{n_w-1}/\partial t\\\partial a_{n_w-1}/\partial t\\\partial \bar{w}_{n_w}/\partial t
\end{bmatrix}
\label{eqn:dr_dt}
\end{equation}
where 
%$\tfrac{\partial \bar{w}_0}{\partial t} = \dot{x} = u$ (as $\bar{w}_0$ is the robot's position by definition),
$\tfrac{\partial \bar{w}_{n_w}}{\partial t} = 0$ ($\bar{w}_{n_w}$ being station's position) and from \eqref{eqn:a_coeff}
\begin{equation}
\begin{bmatrix}
\tfrac{\partial a_0}{\partial t}\\\vdots\\\tfrac{\partial a_{n_w-1}}{\partial t} 
\end{bmatrix}= \Psi^{-1}\begin{bmatrix}
\tfrac{\partial \bar{w}_0}{\partial t}\\0\\\vdots\\0
\end{bmatrix}\Rightarrow \begin{bmatrix}
\tfrac{\partial a_0}{\partial t}\\\vdots\\\tfrac{\partial a_{n_w-1}}{\partial t} 
\end{bmatrix} = \begin{bmatrix}
\psi_0\\\psi_1\\\vdots\\\psi_{n_w-1}
\end{bmatrix}\tfrac{\partial \bar{w}_0}{\partial t}
\label{eqn:da_dt}
\end{equation}
where $\psi_i$ elements are the elements of the first column of $\Psi^{-1}$. Also from \eqref{eqn:b_coeff} 
\begin{equation}
\begin{bmatrix}
\tfrac{\partial b_0}{\partial t}\\\vdots\\\tfrac{\partial b_{n_w-1}}{\partial t}
\end{bmatrix} = \begin{bmatrix}
-\psi_1\\\vdots\\-\psi_{n_w-1}\\-\tfrac{1}{2}\psi_{n_w-1}
\end{bmatrix}\tfrac{\partial \bar{w}_0}{\partial t}
\label{eqn:db_dt}
\end{equation}
and from \eqref{eqn:Rf} we deduce that
\begin{equation}
\scalemath{0.8}{\tfrac{\partial R_n^f}{\partial t} = H_{ff}^{-1}\left(-H_{fc}\begin{bmatrix}
\tfrac{\partial R_{c_1}}{\partial t}\\\tfrac{\partial R_{c_2}}{\partial t}
\end{bmatrix}+\sum_{k=0}^{n_w-1}\Delta\tau_k (S_k^f)^TG_{n,n_k}\begin{bmatrix}
0\\\partial a_k/\partial t\\\partial b_k/\partial t\\0
\end{bmatrix}\right)}
\label{eqn:dRf}
\end{equation}
We note that the lemmas \ref{lemma:base} and \ref{lemma:2} still hold in the same way for the case of varying $R_n$. However, since now $\tfrac{dL}{dt} =-\left|\tfrac{\partial L}{\partial t}\right|\eta+\tfrac{\partial L}{\partial t}$ then \eqref{eqn:eta_r} will become
\begin{equation*}
\eta_r = \frac{v_r+\tfrac{\partial L}{\partial t}}{\left|\tfrac{\partial L}{\partial s}\right|}
\end{equation*}
and following same steps in lemma \ref{lemma:speed_limit} \eqref{eqn:abs_u_ineq} becomes
\begin{equation}
||u||\leq \left|v_r + \tfrac{\partial L}{\partial t}\right|+ \gamma_d\epsilon
\label{eqn:max_lt}
\end{equation} 
To deal with this issue, we introduce a new point $\zeta\in\mathbb{R}^2$ and let it be the head of the Bezier path, i.e. $\bar{w}_0 = \zeta$ instead of $\bar{w}_0= x$ and we control $\zeta$ in the manner described in the next proposition.
\begin{proposition}
	\label{proposition:freeze}
	Consider a robot with dynamics \eqref{eqn:robot_dynamics} applying the proposed energy sufficiency framework described by the CBFs \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound}. Suppose we set $\bar{w}_0 = \zeta$, where $\zeta\in\mathbb{R}^2$ and obeys the dynamics 
	\begin{equation}
	\dot{\zeta} = -K_{\zeta}(\zeta-x)\left(1-\xi(s)\right)
	\label{eqn:p_con}
	\end{equation}
	where $\xi$ is an activation function defined as
	\begin{equation}
%	\xi(s)=\frac{1}{1+e^{K(s-\epsilon_{\zeta})}}
	\xi(s) = \begin{cases}
	0\quad s \leq \sigma\\
	1\quad\text{otherwise}
	\end{cases}
	\end{equation} 
	with  $0<\sigma\ll1$ and $||x-x_r(\sigma)||\ll \epsilon$. Then \eqref{eqn:tracking_cbf} is a ZCBF. 
%	\todo{we can add a condition on $\epsilon$ such that the reference point doesn't get out of the tracking circle around x in hd}
\end{proposition}
\begin{proof}
	Similar to \eqref{eqn:abs_u_ineq}, if the right hand side of \eqref{eqn:max_lt} is less than $||u_{\max}||$ then it means there is always a control action that satisfies \eqref{eqn:tracking_constraint} (with the added $\tfrac{\partial L}{\partial t}$). However if the right hand side of \eqref{eqn:max_lt} is not less than $||u_{\max}||$ (meaning the control action $u$ may saturate), by choosing $\sigma$ arbitrarily small the reference point $x_r$ will still satisfy $h_d > 0$ on the interval $s\in[0,\sigma]$. Moreover, on the interval $s\in\left]\sigma,1\right]$ the activation function $\xi$ will be activated and from  \eqref{eqn:p_con} we get $\dot{\zeta} =\dot{\bar{w}}_0= 0$. Then from \eqref{eqn:da_dt}, \eqref{eqn:db_dt} and \eqref{eqn:dr_dt} we get that $\tfrac{\partial R_n}{\partial t} = 0$, which leads to $\tfrac{\partial f}{\partial t} = 0$ from \eqref{eqn:At} and \eqref{eqn:pf_pt}, which in the end gives $\tfrac{\partial L}{\partial t} = 0$. As a result \eqref{eqn:tracking_inequality} and \eqref{eqn:speed_ineq} hold and same result of lemma \ref{lemma:speed_limit} follows.
\end{proof}

What the last proposition suggests is a method of "freezing" the Bezier path while the robot takes the path back to the station, in which case the same methods proposed in the previous section apply. The QP problem considered so far will be
\begin{equation}
\begin{aligned}
&  \mathbf{u}^*=\underset{\mathbf{u}}{\text{min}}
& & ||\mathbf{u}-\mathbf{u}_{nom}||^2 \\
& \quad \quad \quad \text{s.t.}
& & \mathbf{A}\mathbf{u} \geq \mathbf{B} \\
%&&& X \succeq 0.
\end{aligned}
\label{eqn:QP_suff}
\end{equation}
where 
\begin{equation}
\begin{split}
\mathbf{A} &= \begin{bmatrix}
\tfrac{-{k_e(V-h_e)}}{v_r}G_1 &\mathbf{0}_{1\times 2}\\1&\mathbf{0}_{1\times 2}\\
0&-\tfrac{(x-x_r)^T}{||x-x_r||}
\end{bmatrix}\\ 
\mathbf{B} &= \begin{bmatrix}
-\gamma_e h_e + k_eV+\tfrac{k_e(V-h_e)}{v_r}G_2\\-\gamma_bh_b\\
-\gamma_dh_d-\tfrac{(x-x_r)^T}{||x-x_r||} \dot{x}_r
\end{bmatrix}\\
G_1 &= \tfrac{1}{2}\left[-\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right.\\&\left.+(1-s)\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right]\\
G_2&=\tfrac{1-s}{2}\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial t}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\\
\mathbf{u}_{nom}&=\begin{bmatrix}
-1&u_{nom}
\end{bmatrix}
\end{split}
\label{eqn:defs}
\end{equation}

%\Rightarrow&-k_eV-\frac{k_e}{v_r}(V-h_e)\frac{dL}{dt} \geq -\gamma_e h_e

\begin{theorem}
	\label{thm:suff}
	For a robot described by \eqref{eqn:robot_dynamics} with a set of ordered waypoints $\mathcal{W}\in\mathbb{R}^{n_w\times 2}$ and augmented set of waypoints $\bar{\mathcal{W}} = \begin{bmatrix}
	x^T&\mathcal{W}^T	\end{bmatrix}^T$ and applies \eqref{eqn:a_coeff} and \eqref{eqn:b_coeff} along with \eqref{eqn:Rn} for Bezier path construction, then \eqref{eqn:QP_suff} ensures energy sufficiency is guaranteed.
\end{theorem}
\begin{proof}
	Since \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} are ZCBFs then from lemma \ref{lemma:base} and \ref{lemma:2} and by plugging $\delta_m$ from \eqref{eqn:delta_m} in \eqref{eqn:energy_suff_cbf}, the reference point $x_r$ will arrive to the boundary of the charging region while moving along the Bezier path with a constant speed $v_r$, and given that \eqref{eqn:tracking_cbf} is a ZCBF then the robot is guaranteed to follow the reference point and be inside the charging region while $V\nless V_m$ as shown in proposition \ref{proposition:length_error}. 
\end{proof}
\subsection{Effect of path planning}
During the course of a mission, the path planner keeps updating the waypoints back to the charging station every $\mathcal{T}$ seconds, meaning that there are discrete changes in the number of waypoints and their locations, which can lead to violating \eqref{eqn:energy_suff_cbf}. For that end, we impose some conditions on the output of the path planner so as not to violate other constraints. 
\begin{theorem}
	For a robot described by \eqref{eqn:robot_dynamics} that applies the control strategy in \eqref{eqn:QP_suff} for an already existing set of waypoints $\mathcal{W}^{(k-1)\mathcal{T}}$ at time $(k-1)\mathcal{T}$, $k\in \mathbb{N}$. Suppose a path planner produces a candidate set of waypoints $\mathcal{W}^{k\mathcal{T}}$ at time $k\mathcal{T}$. If the augmented set of waypoints $\bar{\mathcal{W}}^{k\mathcal{T}} = \begin{bmatrix}
	x^T &(\mathcal{W}^{k\mathcal{T}})^T
	\end{bmatrix}^T$ satisfies the next two conditions

	\begin{subequations}
		\begin{equation}
		h_e = V-V_me^{\tfrac{k_e}{v_r}(L(s)-\delta_m)}>0
		\label{eqn:keep_suff}
		\end{equation}
		\begin{equation}
		-k_eV-\frac{k_e}{v_r}(V-h_e)G_2 > -\gamma_e h_e
		\label{eqn:keep_d_suff}
		\end{equation}
		\label{eqn:keep}
	\end{subequations}
	where $G_2$ is as defined in \eqref{eqn:defs}, then energy sufficiency is maintained.
\end{theorem}
\begin{proof}
	If the new set of augmented waypoints satisfy \eqref{eqn:keep_suff} then switching from $\mathcal{W}^{(k-1)\mathcal{T}}$ to $\mathcal{W}^{k\mathcal{T}}$ will not violate the energy sufficiency constraint encoded by $h_e$. Moreover, if said switching satisfies \eqref{eqn:keep_d_suff}, then $h_e > 0$ is satisfied with $s = 0$ (notice that $\tfrac{dL}{dt}= G_1\eta + G_2$), meaning that the reference point $x_r$ will be still tracking the robot's position by virtue of proposition \ref{proposition:freeze}, thus $h_d > 0$ will not be violated as well, and from theorem \ref{thm:suff} energy sufficiency is maintained.
\end{proof}
\begin{remark}
	In case any of the two constraints in \eqref{eqn:keep} is not satisfied, the new set of waypoints will not be admitted and the old set of waypoints $\mathcal{W}^{(k-1)\mathcal{T}}$ can be used and energy sufficiency is maintained by virtue of theorem \ref{thm:suff}. Algorithm \ref{algo} summarizes the main steps discussed above. 
\end{remark}
\begin{algorithm}
	\caption{Admission of new path at time $k\mathcal{T}$}
	\label{algo}
	\begin{algorithmic}
		\Require $\mathcal{W}^{(k-1)\mathcal{T}}$,$\mathcal{W}^{k\mathcal{T}}$, $x$
		\State$\bar{\mathcal{W}}^{k\mathcal{T}} \gets \begin{bmatrix}x^T&(\mathcal{W}^{k\mathcal{T}})^T \end{bmatrix}^T$
		\State $L\gets$ PATH\_LENGTH($\bar{\mathcal{W}}^{k\mathcal{T}}$)
		\If{\eqref{eqn:keep_suff} == False OR \eqref{eqn:keep_d_suff} == False}
			\State $\mathcal{W}^{k\mathcal{T}}\gets \mathcal{W}^{(k-1)\mathcal{T}}$ 
			\State $\bar{\mathcal{W}}^{k\mathcal{T}} \gets \begin{bmatrix}x^T&(\mathcal{W}^{k\mathcal{T}})^T \end{bmatrix}^T$
		\EndIf
		\State \Return $\bar{\mathcal{W}}^{k\mathcal{T}}$
	\end{algorithmic}
\end{algorithm}
In algorithm \ref{algo} PATH\_LENGTH($\bar{\mathcal{W}}^\mathcal{T}$) is a procedure that takes a set of augmented waypoints, does the Bezier segment interpolation as described in \eqref{eqn:a_coeff} and \eqref{eqn:b_coeff}, merges these segments according to \eqref{eqn:Rn}, and finally return the length of the merged curve as described in \eqref{eqn:bez_len}.

==> figures/Sim/tex_fig/trajectory_plot.tex <==
\tikzset{
  %Define style for boxes
  box1/.style={
           rectangle,
           draw=black, 
           thick,
           text centered},
    %Define standard arrow tip
    >=stealth',
    % Define arrow style
    arrow1/.style={
           %->,
           thick,
           shorten <=2pt,
           shorten >=2pt,
           }
}
\definecolor{eblue}{rgb}{0, 0, 0.8}
\definecolor{rred}{rgb}{0.8, 0, 0}
\definecolor{hgreen}{rgb}{0, 0.6, 0}
\definecolor{chbrown}{rgb}{0.6,0.298039216, 0}
\definecolor{torange}{rgb}{1,0.501960784, 0}
\definecolor{pviolet}{rgb}{0.533333333, 0.454901961, 0.764705882}
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

\begin{figure}[!htb]
\centering
    \begin{tikzpicture}
    
	\begin{axis}[
		width = 1.5\columnwidth,
		height = 28cm,
		xmin=0,
		xmax=100,
		ymin=0,
		ymax=100,	
		%grid=both,
		grid=none,
		axis line style={draw=none},
		tick style={draw=none},
		xticklabel=\empty,
		yticklabel=\empty,
		]
	
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\begin{pgfonlayer}{main}

% Legend 

\node at (axis cs:37.5,97) (nd2) {\includegraphics[scale=0.4,width=14.4cm]
{../Map_figures/legend_raw.pdf}}; 

	\node 
		at (axis cs:16.8,98.3) 
		(exp_leg) { \textcolor{black}{Exploration R1}};

	\node 
		at (axis cs:15.4,95.8) 
		(exp_leg1) { \textcolor{black}{Homing R1}};
		
	\node 
		at (axis cs: 40.2,98.3) 
		(exp_leg1) { \textcolor{black}{Exploration R2}};

	\node 
		at (axis cs:38.8,95.8) 
		(exp_leg1) { \textcolor{black}{Homing R2}};
		
	\node 
		at (axis cs: 61,98.3) 
		(exp_leg1) { \textcolor{black}{Obstacles}};

	\node 
		at (axis cs:63.7,95.8) 
		(exp_leg1) { \textcolor{black}{Charging Station}};

% Figures 


\node at (axis cs:54,80) (nd2) {\includegraphics[scale=0.4,width=7.6cm]
{../Map_figures/HHir_indoor_maze_maze512-32-4_30_exp_2_12.pdf}}; 
\node at (axis cs:18,80) (nd1) {\includegraphics[scale=0.4,width=7.6cm]
{../Map_figures/HHir_indoor_maze_maze512-32-2_30_exp_2_13.pdf}};


%\node at (axis cs:74,58) (nd6) {\includegraphics[scale=0.35,width=6cm]
%{../Map_figures/maze-2_13_kh50.png}};
\node at (axis cs:56,58) (nd5) {\includegraphics[scale=0.4,width=7cm]
{../Map_figures/maze-4_12_kh50.png}}; 
\node at (axis cs:20,58) (nd4) {\includegraphics[scale=0.4,width=7cm]
{../Map_figures/maze-2_13_kh50.png}};

\node at (axis cs:54,35) (nd7) {\includegraphics[scale=0.4,width=7.6cm]
{../Map_figures/HHir_indoor_maze_maze512-32-8_30_exp_2_13.pdf}}; 
\node at (axis cs:18,35) (nd6) {\includegraphics[scale=0.4,width=7.6cm]
{../Map_figures/HHir_indoor_maze_maze512-32-6_30_exp_2_12.pdf}}; 


\node at (axis cs:56,13) (nd9) {\includegraphics[scale=0.4,width=7cm]
{../Map_figures/maze-8_13_kh50.png}};
\node at (axis cs:20,13) (nd8) {\includegraphics[scale=0.4,width=7cm]
{../Map_figures/maze-6_12_kh50.png}};20

%\node at (axis cs:12,15) (nd13) %{\includegraphics[scale=0.35,width=5cm]
%{../Plots/sim_cmp_target_reached_result}};
% Names

		
	
	\node 
		at (axis cs:0.8,93) 
		(nd_exp) {\large \textcolor{black}{\textbf{A}}};
		
	\node 
		at (axis cs:37,93) 
		(nd_exp) {\large \textcolor{black}{\textbf{B}}};

	\node 
		at (axis cs:1,64.5) 
		(nd_exp) {\large \textcolor{black}{\textbf{C}}};
		
	\node 
		at (axis cs:38,64.5) 
		(nd_exp) {\large \textcolor{black}{\textbf{D}}};
		

	\node 
		at (axis cs:0.8,49) 
		(nd_exp) {\large \textcolor{black}{\textbf{E}}};
		
	\node 
		at (axis cs:37,49) 
		(nd_exp) {\large \textcolor{black}{\textbf{F}}};

	\node 
		at (axis cs:1,19.5) 
		(nd_exp) {\large \textcolor{black}{\textbf{G}}};
		
	\node 
		at (axis cs:38,19.5) 
		(nd_exp) {\large \textcolor{black}{\textbf{H}}};
		
		

\end{pgfonlayer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Horizontal boxes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{pgfonlayer}{background}
 

%\end{pgfonlayer}



	\end{axis}	
	
    \end{tikzpicture}
    
\caption{Figure caption.}
\label{fig:diagram2} 
\end{figure}


==> figures/Sim/tex_fig/trajectory_plot_new.tex <==
\tikzset{
  %Define style for boxes
  box1/.style={
           rectangle,
           draw=black, 
           thick,
           text centered},
    %Define standard arrow tip
    >=stealth',
    % Define arrow style
    arrow1/.style={
           %->,
           thick,
           shorten <=2pt,
           shorten >=2pt,
           }
}
\definecolor{eblue}{rgb}{0, 0, 0.8}
\definecolor{rred}{rgb}{0.8, 0, 0}
\definecolor{hgreen}{rgb}{0, 0.6, 0}
\definecolor{chbrown}{rgb}{0.6,0.298039216, 0}
\definecolor{torange}{rgb}{1,0.501960784, 0}
\definecolor{pviolet}{rgb}{0.533333333, 0.454901961, 0.764705882}
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

\begin{figure}[!htb]
\centering
    \begin{tikzpicture}
    
	\begin{axis}[
		width = 1.5\columnwidth,
		height = 28cm,
		xmin=0,
		xmax=100,
		ymin=0,
		ymax=100,	
		%grid=both,
		grid=none,
		axis line style={draw=none},
		tick style={draw=none},
		xticklabel=\empty,
		yticklabel=\empty,
		]
	
		
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
\begin{pgfonlayer}{main}

% Legend 



% Figures 


\node at (axis cs:54,80) (nd2) {\includegraphics[scale=0.4,width=7.6cm]
{../June_map_figures/maze4_2.png}}; 
\node at (axis cs:18,80) (nd1) {\includegraphics[scale=0.4,width=7.6cm]
{../June_map_figures/HHir_indoor_maze_maze512-32-4_30_exp_2_2.pdf}};

%\node at (axis cs:12,15) (nd13) %{\includegraphics[scale=0.35,width=5cm]
%{../Plots/sim_cmp_target_reached_result}};
% Names

		
	
	\node 
		at (axis cs:0.8,93) 
		(nd_exp) {\large \textcolor{black}{\textbf{A}}};
		
	\node 
		at (axis cs:37,93) 
		(nd_exp) {\large \textcolor{black}{\textbf{B}}};

	
		

\end{pgfonlayer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Horizontal boxes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{pgfonlayer}{background}
 

%\end{pgfonlayer}



	\end{axis}	
	
    \end{tikzpicture}
    
\caption{Figure caption.}
\label{fig:diagram2} 
\end{figure}


==> introduction.tex <==
Robotics and artificial intelligence is alleviating the workload on humans and, most importantly, enabling deployments in hazardous environments and saving lives. Exploration of unknown and potentially dangerous environments is typical task robots perform in terrestrial~\cite{best2022resilient} and extraterrestrial~\cite{bajracharya2008autonomy} applications. Terrestrial applications demanding exploration include search and rescue~\cite{balta2017integrated}, construction~\cite{yang2021hallway}, and mining~\cite{thrun2004autonomous}. Furthermore, hundreds of subsurface environments (caves) have been sited on the lunar surface and the Martian terrain~\cite{cushing2012candidate}, which remains to be explored. Exploration of subsurface environments on extraterrestrial bodies is vital because of its potential to identify life beyond Earth and discover radiation-shielded locations to host humans~\cite{titus2021science}. These application scenarios have motivated the design of many exploration planners for robots~\cite{morrell2022nebula, dang2019graph}. In many of these approaches, one crucial component that must be deployed on the robots to enable long-term autonomy is a method to replenish the robot batteries on time. Delays in charging the battery that extend a specific window will render the robot useless, consider exploration of lava tubes on the lunar surface; robots need to exit the cave and get to a location with sunlight to recharge before exploring further when the battery is low. In many of these applications, communication with the robot is impractical or non-feasible to monitor the battery levels and instruct the robot to a charging station~\cite{miaja2022robocrane}.

\begin{figure}[!htb]
	\centering
	\includegraphics[width=\columnwidth]{figures/rover_figures/pointclod_image}
    \caption{Maintaining energy sufficiency during the exploration of a corridor environment.}
	\label{fig:rover_explore}
\end{figure}

During an exploration mission, one straightforward approach to maintaining energy sufficiency (maintaining the required energy levels on the robot) is to set an energy threshold to return to a charging point or at the end of a mission session~\cite{tranzatto2022team}. However, in many realistic long-term deployments, such an approach cannot guarantee energy sufficiency and render the robot without energy before reaching a charging point. Some challenges with harsh unstructured environments are imperfect robot localization, traversing uneven rough terrains consuming varying amounts of power and alleviating traversal times, and increased traversal time due to complex environmental structures. Methods to maintain energy sufficiency should be capable of handling these challenges while guaranteeing that the robot will never run out of energy (maintain energy sufficiency). 

A wide range of methodologies has been investigated in the literature to achieve this goal, like using static charging stations~\cite{notomista2018persistification,ravankar2021multi,liu2014optimal}, moving charging stations that do rendezvous with the mission robots to recharge them or swap their batteries~\cite{mathew2015multirobot,kundu2021mobile,kamra2017combinatorial}, or deposit full batteries along robot's mission path~\cite{ding2019decentralized}. Many of these approaches do not provide guarantees on energy sufficiency or cannot tackle harsh unstructured environments. Some methods~\cite{alizadeh_optimized_2014,fu_targeted_2019,schneider2014electric} formulate the energy sufficiency problem as a combinatorial optimization with the environment treated as a weighted graph encoding energy costs, travel times, and travel distances. The main shortcoming of these methods is that the computation complexity increases rapidly for large environments. These methods also require a map of the environment beforehand and cannot be used in an exploration mission. Another body of works applies heuristics like Genetic Algorithms (GA) \cite{li2018planning}, Tabu-Search (TS) \cite{wang_staying-alive_2008} and Monte Carlo Tree Search (MCTS)\cite{warsame2020energy} to the graph formulation to alleviate the computational complexity but still suffer from the need for a map of the environment. 

In a typical exploration mission, the robot proceeds in a receding horizon with the environment only perceived up to the sensors' field of view. Based on the information in hand thus far, the robot makes choices on trajectories to maximize environmental coverage. Several well-designed exploration planners exist in the literature developed within or outside the scope of the DARPA SubTerranian challenge~\cite{subt_challenge}. A few such planners are a graph-based exploration planner (GbPlanner~\cite{dang2019graph}), Next-Best-View planner~\cite{bircher2016receding}, Motion primitives-based planner (MbPlanner~\cite{dharmadhikari2020motion}), Dual-Stage Viewpoint Planner~\cite{zhu2021dsvp}, and TARE planner~\cite{cao2021tare}. These planners can produce an exploration trajectory and a trajectory back to any point in the map, given odometry and a map of the environment incrementally built thus far. Even though these planners are robustly constructed and can efficiently handle the challenges created by unstructured environments, they still need to equip a mission planning module that can guarantee energy sufficiency to enable long-term autonomy. 

In this work, we design a modular and mission-agnostic method that uses a control barrier function to guarantee energy sufficiency when applied alongside any arbitrary exploration planner. The approach builds upon our previous work \cite{fouad2020energy}, and \cite{fouad2022energy}, which provides energy-sufficiency guarantees for robots in simpler environments. We thus extend our previous efforts to validate energy autonomy guarantees on generic obstacle-free paths generated by path planners. The modular approach applies to a wide range of applications that employ a path planner,  especially the exploration of unknown subterranean environments~\cite{dang2019graph}, navigation in urban~\cite{mehta2015human,ramana2016motion}, and indoor environments~\cite{zhao2013path}.

\todo[inline]{Hassan: make sure what I say bellow makes sense and it is the best way to briefly explain our method.}

The main principle behind the method is a control barrier function that encodes the energy-sufficiency requirements and periodically queries a path planner to obtain a path back to the charging station, estimating energy requirements to reach a recharge point. When the energy requirements are sufficient to reach a charging station, the robot performs its mission; otherwise, it is directed to a charging station. We leverage the properties of a control barrier function across a bezier path to guarantee energy sufficiency on the robot at all times. We evaluate our method at first using a large-scale simulation in a set of maze environments and perform experiments on experimental hardware executing exploration in a real-world corridor environment. The importance of our result is that we observe energy sufficiency fulfillment at all times during any given mission, both in simulation and hardware.

The paper is organized as follows: sec.~\ref{sec:related_work} reviews the literature around energy sufficiency, awareness in path planning, and some relevant topics to our frameworks like path smoothing and control barrier functions (CBFs); sec.~\ref{sec:background} presents the required preliminaries to our formulation; sec.~\ref{sec:static} introduces the method considering a particular case with robot being stationary and path non-changing; sec.~\ref{sec:dynamic} extends the previous section presenting the method for moving robots and path updates as the robot moves; sec.~\ref{sec:results} shows simulation and hardware results; and sec.~\ref{sec:conc} provides some concluding remarks, lessons learned and future works.

%One important feature that needs to be present in a functional energy sufficiency methodology is the ability to function in unstructured and cluttered environments like spaces with obstacles~\cite{li2018planning} and urban environments~\cite{schneider2014electric,desaulniers2016exact}. Typically, the problem of driving the robot back during mission execution to recharge in a generic environment is formulated as a combinatorial optimization problem where the environment is modeled as a weighted graph, with vertices representing locations of interest and edges with weights that encode different types of costs like energy costs, travel times and travel distances to give a few examples \cite{fu_targeted_2019,alizadeh_optimized_2014,schneider2014electric}. Some heuristic solutions for such graph formulations are also employed like Genetic Algorithms (GA) \cite{li2018planning}, Tabu-Search (TS) \cite{wang_staying-alive_2008} and Monte Carlo Tree Search (MCTS)\cite{warsame2020energy}.

%\textcolor{red}{The main drawbacks of such techniques are the relative computational complexity for solving such optimization problems and the additional overhead of accurate environment modeling, i.e. the need to knowing the nodes and the edge weights beforehand, which makes such methods less flexible for a wide variety of applications like exploration missions, in which such graphs may not be readily available. Variants of Rapidly-exploring Random Tree (RRT) method, on the other hand, provide  sampling based planning that merges the path finding and the environment construction processes, thus eliminating the need for \emph{a-priori} structured representation of environment\cite{souissi2013path}. Moreover, such methods are generally fast and provide Asymptotic Optimality.}

%In this work we present a mission agnostic energy sufficiency layer that can be applied alongside a sample based path planner (e.g. RRT*) to navigate unstructured environments maintaining required energy levels. We mean by energy sufficiency that a robot does not consume more energy than an allocated energy budget. In previous work \cite{fouad2020energy} and \cite{fouad2022energy} our proposed framework is capable of providing energy sufficiency guarantees for robots in simple environments, such that a robot's path back to the charging station is a straight line. 

%We thus extend our previous results to validate energy autonomy guarantees on generic obstacle free paths generated by path planners. Our proposed approach is attractive for a wide range of applications that use sampling based path planners, especially exploration of unknown subterranean environments \cite{dang2019graph}, navigation in urban environments \cite{mehta2015human,ramana2016motion}, and indoor navigation \cite{zhao2013path}.

%\textcolor{blue}{In this work, we take a path produced by a sampling based planner in the form of waypoints, then we use double sigmoid functions to create a smoother representation of this path, and we modify our framework from \cite{fouad2022energy} to enable the robot to slide along the obtained smooth path in a manner that ensures energy sufficiency as defined earlier.}

% The layout of the paper is as follows. In section \ref{sec:related_work} we review the literature that relates to energy sufficiency and awareness in path planning, as well as some relevant topics to our framework as path smoothing and control barrier functions (CBFs). In section \ref{sec:background} we give some preliminaries and we present the problem definition. In section \ref{sec:static} we pave the way for presenting our proposed energy sufficiency framework by considering the special case when the robot is static and the path is non-changing. In section \ref{sec:dynamic} we build on results from the previous section to consider the general case of a moving robot and path updates from the path planner. In section \ref{sec:results} we present our simulation and hardware results and we give some concluding remarks in section \ref{sec:conc}.


==> proposition_2.tex <==
\begin{proposition}
	\label{proposition:freeze}
	Consider a robot with dynamics \eqref{eqn:robot_dynamics} applying the proposed energy sufficiency framework described by the CBFs \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound}. Suppose we set $\bar{w}_0 = \zeta$, where $\zeta\in\mathbb{R}^2$ and has the dynamics 
	\begin{equation}
	\dot{\zeta} = -K_{\zeta}(\zeta-x)\left(1-\xi(s)\right)
	\label{eqn:p_con}
	\end{equation}
	where $\xi$ is an activation function defined as
	\begin{equation}
%	\xi(s)=\frac{1}{1+e^{K(s-\epsilon_{\zeta})}}
	\xi(s) = \begin{cases}
	0\quad s \leq \sigma\\
	1\quad\text{otherwise}
	\end{cases}
	\end{equation} 
	with   $0<\sigma\ll1$ and $||x-x_r(\sigma)||\ll \epsilon$, then \eqref{eqn:energy_suff_cbf} and \eqref{eqn:tracking_cbf} are ZCBF.
%	Then energy sufficiency is maintained.
%	Then \eqref{eqn:tracking_cbf} is a ZCBF. 
%	\todo{we can add a condition on $\epsilon$ such that the reference point doesn't get out of the tracking circle around x in hd}
\end{proposition}
\begin{proof}
We start by noting that \eqref{eqn:p_con} achieves tracking of robot's position in case $s=0$, with an error inversely proportional to $K_\xi$. This could be shown with the candidate Lyapunov function 
\begin{equation}
V = \tfrac{1}{2}(x-\xi)^T(x-\xi), \quad \dot{V} = (x-\xi)^Tu-K_\xi||x-\xi||^2
\end{equation} 
which has $\dot{V}\leq0$ under high value of $K_\xi$ (which is feasible since $\xi$ is an imaginary point with no physical characteristics). 
Moreover, since $\eta\in\mathbb{R}$ then there is a value of $\eta$ capable of satisfying the following inequality
	\begin{equation}
	\begin{split}
	&\eta \geq \tfrac{1}{||R_{n}^TB^T T^\prime(s)||}\left(\tfrac{\mathcal{P}(u)-\gamma_eh_e}{\mathcal{P}(v_r)}v_r+\tfrac{\partial L}{\partial t}\right)
	\end{split}
	\label{eqn:suff_const_dyn}
	\end{equation}
	 which is \eqref{eqn:suff_constraint} with the additional $\tfrac{\partial L}{\partial t}$ term.  If $\eta_{nom}$ satisfies \eqref{eqn:suff_const_dyn} then $u = u_{nom}$ (as long as \eqref{eqn:tracking_constraint} is satisfied). We point out that under $u_{nom}$ $\tfrac{\partial L}{\partial t} < 0$ when $\tfrac{d}{dt}||\xi-\bar{w}_{1} |||< 0$, i.e. the head of the Bezier path approaches its following waypoint (the interpolating cubic Bezier segment between $\bar{w}_0$ and $\bar{w}_1$ will need to shrink to maintain its free end condition). 
	 
	 When $\eta_{nom}$ violates \eqref{eqn:suff_const_dyn}, a safe value of $\eta$ is that achieving equality in \eqref{eqn:suff_const_dyn}
	 
	 Initially when $s=0$ and  $h_e\rightarrow 0$, i.e. approaches the boundary of the its safe set and the nominal value of $\eta = 0$ does not satisfy \eqref{eqn:suff_const_dyn}, a safe $\eta$ achieves the equality of \eqref{eqn:suff_const_dyn}  
	\begin{equation}
	\eta = \tfrac{1}{||R_{n}^TB^T T^\prime(s)||}\left(\tfrac{\mathcal{P}(u)}{\mathcal{P}(v_r)}v_r+\tfrac{\partial L}{\partial t}\right)
	\label{eqn:suff_equality}
	\end{equation}
	and as long as  $u$ in \eqref{eqn:suff_const_dyn} does not violate \eqref{eqn:tracking_constraint} then $u=u_{nom}$. If $\eta_{nom} = 0$ then $\eta > 0$ in \eqref{eqn:suff_equality} so $s$ will increase. 
%	(since \eqref{eqn:tracking_cbf} is the only CBF that has access to controlling $u$)
%	 Unless $u_{nom}$ is causing $\tfrac{\partial L}{\partial t} <0$  (meaning $h_e$ would be increasing and the system would be moving further into its safe set and in this case \eqref{eqn:suff_const_dyn} is invalid) in which case 
%	
%	
%	
%	 
%	Similar to \eqref{eqn:abs_u_ineq}, if the right hand side of \eqref{eqn:max_lt} is less than $||u_{\max}||$ then it means there is always a control action that satisfies \eqref{eqn:tracking_constraint} (with the added $\tfrac{\partial L}{\partial t}$). However if the right hand side of \eqref{eqn:max_lt} is not less than $||u_{\max}||$ (meaning the control action $u$ may saturate), by choosing $\sigma$ arbitrarily small the reference point $x_r$ will still satisfy $h_d > 0$ on the interval $s\in[0,\sigma]$. Moreover, on the interval $s\in\left]\sigma,1\right]$ the activation function $\xi$ will be activated and from  \eqref{eqn:p_con} we get $\dot{\zeta} =\dot{\bar{w}}_0= 0$. Then from \eqref{eqn:da_dt}, \eqref{eqn:db_dt} and \eqref{eqn:dr_dt} we get that $\tfrac{\partial R_n}{\partial t} = 0$, which leads to $\tfrac{\partial f}{\partial t} = 0$ from \eqref{eqn:At} and \eqref{eqn:pf_pt}, which in the end gives $\tfrac{\partial L}{\partial t} = 0$. As a result \eqref{eqn:tracking_inequality} and \eqref{eqn:speed_ineq} hold and same result of lemma \ref{lemma:speed_limit} follows.
\end{proof}

==> proposition_2_simple.tex <==
\begin{proposition}
	\label{proposition:freeze}
	Consider a robot with dynamics \eqref{eqn:robot_dynamics} applying the proposed energy sufficiency framework described by the CBFs \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound}. Suppose we set $\bar{w}_0 = \zeta$, where $\zeta\in\mathbb{R}^2$ and has the dynamics 
	\begin{equation}
	\dot{\xi} = -K_{\xi}(\xi-x)\left(1-\zeta(s)\right)
	\label{eqn:p_con}
	\end{equation}
	where $\xi$ is an activation function defined as
	\begin{equation}
	%	\xi(s)=\frac{1}{1+e^{K(s-\epsilon_{\zeta})}}
	\zeta(s) = \begin{cases}
	0\quad s \leq \sigma\\
	1\quad\text{otherwise}
	\end{cases}
	\end{equation} 
	with   $0<\sigma\ll\bar{\sigma}<1$ and $||\xi-x_r(\bar{\sigma})||= \epsilon$, then \eqref{eqn:energy_suff_cbf} and \eqref{eqn:tracking_cbf} are ZCBF.
	%	Then energy sufficiency is maintained.
	%	Then \eqref{eqn:tracking_cbf} is a ZCBF. 
	%	\todo{we can add a condition on $\epsilon$ such that the reference point doesn't get out of the tracking circle around x in hd}
\end{proposition}
\begin{proof}
	We start by noting that \eqref{eqn:p_con} achieves tracking of robot's position in case $s=0$, with an error inversely proportional to $K_\xi$. This could be shown with the candidate Lyapunov function 
	\begin{equation}
	V = \tfrac{1}{2}(x-\xi)^T(x-\xi), \quad \dot{V} = (x-\xi)^Tu-K_\xi||x-\xi||^2
	\end{equation} 
	which has $\dot{V}\leq0$ under high value of $K_\xi$ (which is feasible since $\xi$ is an imaginary point with no physical characteristics). 
	Moreover, since $\eta\in\mathbb{R}$ then there is a value of $\eta$ capable of satisfying the following inequality
	\begin{equation}
	\begin{split}
	&\eta \geq \tfrac{1}{||R_{n}^TB^T T^\prime(s)||}\left(\tfrac{\mathcal{P}(u)-\gamma_eh_e}{\mathcal{P}(v_r)}v_r+\tfrac{\partial L}{\partial t}\right)
	\end{split}
	\label{eqn:suff_const_dyn}
	\end{equation}
	which is \eqref{eqn:suff_constraint} with the additional $\tfrac{\partial L}{\partial t}$ term. In this proof we consider that $\eta_{nom}=0$, which if violates \eqref{eqn:suff_const_dyn}, taking the equality of \eqref{eqn:suff_const_dyn} maintains safety and this implies $\eta\geq0$ ($s$ increases and $x_r$ moves along the path). As a result $h_d$ in \eqref{eqn:tracking_cbf} will approach the boundary of its safe set (in the limiting case $||\xi-x_r|| = \epsilon$ at $s=\bar{\sigma}$, noticing that $\xi$ tracks $x$ as pointed out earlier). Since $s(t)$ is continuous and $\sigma \ll \bar{\sigma}$ this implies that $\dot{\xi} = 0$ before $s(t) = \bar{\sigma}$ , making the Bezier path static before $h_d$ approaches the boundary of its safe set (i.e. $||x-x_r||\approx \epsilon$), thus the result of lemma \ref{lemma:base} follows.  
\end{proof}


\begin{remark}
	The previous treatment was carried out considering $\eta_{nom}=0$ for simplification, but the same conclusion is valid for $\eta_{nom} < 0$. The main idea is to show that the right hand side of \eqref{eqn:suff_const_dyn} will become positive, for which the inequality will not hold for $\eta_{nom}<0$. As the system goes closer to the boundary of the safe set (i.e. $h_e \ll$), $\tfrac{\mathcal{P}(u)}{\mathcal{P}(v_r)}v_r>0$ by definition, and it can be shown that the sign of $\tfrac{\partial L}{\partial t}$ depends on the sign of $\tfrac{d}{dt}||\xi-\bar{w}_1||=\tfrac{d}{dt}||\bar{w}_0-\bar{w}_1||$. This is because the corresponding interpolating cubic Bezier segment will need to shrink or expand to maintain the free end condition in \eqref{eqn:term_cond}. Consequently even if $\tfrac{\partial L}{\partial t}<0$ 
	(even to satisfy \eqref{eqn:suff_const_dyn})
	 it will be until $ ||\xi-\bar{w}_1||\ll$ to have the right hand side of \eqref{eqn:suff_const_dyn}) greater than zero eventually.
\end{remark}

==> result.tex <==
\subsection{Simulation results}
We present herein the simulation results that highlight the ability of our proposed framework to ensure energy sufficiency in a cluttered environment while coordinating the use of a shared station.

In our simulation setup we use  ARGoS simulator \cite{pinciroli2012argos} as a simulation environment, where a group of KheperaIV robots are running a \sout{frontier exploration} \vivektodo{I would go with ``graph based exploration`` or exploration} and mapping task. Each robot is running an exploration software stack that is capable of using sensory input from a lidar to build a map of a cluttered environment. We use the city map benchmarks from \cite{sturtevant2012benchmarks} as a blueprint for obstacles in the environment, and each map is scaled so that it fits a square of $30\times 30$ meters. We use a group of 8 robots and each robot explores the unexplored portions of the map in a manner that maximizes the volumetric gain \cite{dang2019graph}, i.e. the robots go in directions that maximize the explored regions. Figure~\ref{fig:map} shows an example of a simulation environment based on a map from \cite{sturtevant2012benchmarks}.

\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/map2}
	\caption{Example environment built based on one of the maps from \cite{sturtevant2012benchmarks}, with robots in the middle of the map.}
	\label{fig:map}
\end{figure}

We run 10 groups of experiments for ten different maps from \cite{sturtevant2012benchmarks}, and for each case we run 30 simulations. In each run the robots explore the environment while building a map and using a RRT* to produce a path back to the charging station, located at the origin of the map. We measure the error between the difference in arrival times among every two consecutive arrivals in each charging cycle, and the desired separation in arrival times $\delta_t$. Figure~\ref{fig:box} shows a box plot of the aforementioned errors. \vivektodo{I would add units to the errors in the figure}

\begin{figure}[!htb]
	\centering
	\includegraphics[width=\linewidth]{figures/results/box_1.eps}
	\caption{Boxplot representing the errors between every two consecutive arrivals and the desired separation in arrival times for a group of 10 simulation groups with different maps, each with 30 simulations.}
	\label{fig:box}
\end{figure}

==> static1.tex <==
We start introducing our approach by considering the case when a robot is situated on the head of a fixed Bezier curve (where $\tau=0$) and we show how to modify the energy sufficiency method used in \cite{fouad2020energy} to drive the robot back to the end of the curve ($\tau = 1$) where the charging station is located.

The solution strategy we are adopting is to define a moving reference point $x_r\in\mathbb{R}^2$ on the Bezier curve whose location is defined by  
\begin{equation}
x_r(s) = (T^T(s) B P_c)^T = P_{c}^{T}B^TT(s)
\label{eqn:ref_pt}
\end{equation}
with the progression parameter $s\in[0,1]$. The value of $s$ is controlled so that it approaches the end of curve (where the charging station is located) in a manner that maintains energy sufficiency (i.e. $V\geq V_{\min}$ as the robot moves along the path). For that we assume $s$ changes according to the following relation
\begin{equation}
\dot{s} = \eta
\end{equation}
for $\eta\in\mathbb{R}$ and we use $\eta$ as a part of constraint that drives $x_r$ back to the end of the Bezier path.
We then enforce a constraint on the distance between the robot and this reference point to ensure that the robot actually follows $x_r$ back to the charging station at the right time.

The candidate CBF we are using for energy sufficiency is 
\begin{equation}
h_e = V - V_{\min} - \frac{k_e}{v_r}(L - \delta)
\label{eqn:energy_suff_cbf}
\end{equation}
where $v_r$ is the desired velocity with which the robot moves along the path, $\delta$ is the distance of the boundary of charging region away from its center, noting that the center of the charging region is on the Bezier path at $s = 1$, and $L$ is the distance along the Bezier path from the robot's position till its end and is defined in \eqref{eqn:bez_len}.

The constraint $\dot{h}_e\geq -\alpha(h_e)$ associated with this candidate CBF is 
\begin{equation}
\underbrace{-k_e-\frac{k_e}{v_r}\frac{dL}{dt}}_{\dot{h}_e} \geq -\gamma_e h_e
\label{eqn:suff_constraint}
\end{equation}
where 
\begin{equation}
\begin{split}
\frac{dL}{dt} &= \frac{\partial L}{\partial s}\frac{ds}{dt}= \frac{\eta}{2}\left[-\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right.\\&\left.+(1-s)\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right]
\end{split}
\label{eqn:dL}
\end{equation}
to find $\tfrac{\partial f}{\partial s}$, we define 
\begin{equation}
\begin{split}
A_i &= T^{\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})BP_c\\
A_{i}^{\prime} &=\tfrac{1-\tau_i}{2} T^{\prime\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})BP_c
\end{split}
\label{eqn:A}
\end{equation}
with $T^{\prime}(s)$ defined in \eqref{eqn:t_prime}, and 
\begin{equation}
\frac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = \tfrac{1}{||A||}AA^{\prime^T}
\label{eqn:pf_ps}
\end{equation}
noting that $A\in\mathbb{R}^{1\times 2}$ and that $f(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = ||A||$. The constraint in \eqref{eqn:suff_constraint} leads to changing the value of $s$ (by controlling $\eta$) and thus changing $x_r$ along the Bezier path. We use the following candidate CBF that bounds the value of $s$ from below so that $s\geq 0$
\begin{equation}
h_b = s
\label{eqn:lower_bound}
\end{equation} 
with the associated constraint 
\begin{equation}
\eta \geq -\gamma_bh_b
\label{eqn:lowe_bound_constraint}
\end{equation}
We compliment \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} with another candidate CBF that aims at making the robot follow $x_r$ as it changes, and is defined as follows
\begin{equation}
h_d = \epsilon - ||x-x_r||
\label{eqn:tracking_cbf}
\end{equation} 
with $0<\epsilon\ll 1$. The constraint associated with this candidate CBF is 
\begin{equation}
-\tfrac{(x-x_r)^T}{||x-x_r||}(u-\dot{x}_r)\geq -\gamma_d h_d
\label{eqn:tracking_constraint}
\end{equation}
where 
\begin{equation}
\dot{x}_r = P_{c}^{T}B^TT^{\prime}(s)\eta
\label{eqn:ref_pt_speed}
\end{equation}

In the following lemmas we show that the proposed CBFs thus far will lead the robot to arrive back to the charging station with $V\geq V_{\min}$. 

\begin{lemma}
	\label{lemma:base}
	For a robot with dynamics described in \eqref{eqn:robot_dynamics}, the control barrier functions defined in \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} are zeroing control barrier functions (ZCBF). Moreover, satisfying \eqref{eqn:suff_constraint} leads $x_r$ to move along the path with speed equal to $v_r$.
\end{lemma}
\begin{proof}
	Since $\eta\in\mathbb{R}$, then there exists a value of $\eta$ that satisfies both \eqref{eqn:suff_constraint} and \eqref{eqn:lowe_bound_constraint} separately. We just need to show that both constraints are not contradicting. The inequality \eqref{eqn:suff_constraint} can be rewritten as 
	\begin{equation}
	\frac{dL}{ds}\frac{ds}{dt}=\frac{dL}{ds} \eta\leq \frac{v_r(\gamma_eh_e-k_e)}{k_e}
	\end{equation} 
	but we note that $\tfrac{dL}{ds} < 0$ by definition (i.e. as we go along the path, the remaining path length decreases), thus the last inequality can be rewritten as 
	\begin{equation}
	\begin{split}
	&-\left|\frac{dL}{ds}\right|\eta\leq \frac{v_r(\gamma_eh_e-k_e)}{k_e}\\& \Rightarrow \eta\geq- \frac{v_r(\gamma_eh_e-k_e)}{k_e\left|\tfrac{dL}{ds}\right|}
	\end{split}
	\label{eqn:modified_he_constraint}
	\end{equation}
	therefore there is always a value of $\eta$ that satisfies \eqref{eqn:lowe_bound_constraint} and \eqref{eqn:modified_he_constraint} simultaneously, thus both \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} are both ZCBF.
%	which can be done by noting that since $s$ is a progression parameter for the Bezier path, it should belong to $[0,1]$, meaning that \eqref{eqn:lowe_bound_constraint} is a redundant constraint intended to mathematically restrain $s$ from going below zero.
\end{proof}
Based on the previous result, the constraint \eqref{eqn:suff_constraint} will lead the reference point $x_r$ to move along the Bezier path with a certain speed, as discussed in the next lemma
\begin{lemma}
	\label{lemma:2}
	For a robot with dynamics \eqref{eqn:robot_dynamics} and applying the constraints \eqref{eqn:suff_constraint} and \eqref{eqn:lower_bound}, the reference point $x_r$ along the Bezier path (defined in \eqref{eqn:ref_pt}) moves along the Bezier path back to the charging station such that $\tfrac{dL}{dt} \approx -v_r$.
\end{lemma}
\begin{proof}
Since the equality portion of  \eqref{eqn:suff_constraint} is activated when \eqref{eqn:suff_constraint} is violated by $u_{nom}$, we can consider the equality portion of \eqref{eqn:suff_constraint} which gives 
\begin{equation*}
h_e(t) = h_{e_0}e^{-\gamma_et}
\end{equation*}	
by differentiating both sides we get
\begin{equation}
\begin{split}
&-k_e-\frac{k_e}{v_r}\frac{dL}{dt}= -\gamma_eh_{e_0}e^{-\gamma_et}\\
&\Rightarrow\frac{dL}{dt} = -v_r +\frac{\gamma_ev_r}{k_e}h_{e_0}e^{-\gamma_et}
\end{split}
\end{equation}
we note that the last term can be made arbitrarily small by choosing $\gamma_e$ to be arbitrarily high.
\end{proof}


\begin{lemma}
	Given a robot with dynamics as described in \eqref{eqn:robot_dynamics}, has a limited control effort $||u||\leq||u_{\max}||$ and adopting the CBFs in \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound}, and provided that $v_r+\gamma_d\epsilon\leq||u_{\max}||$, then \eqref{eqn:tracking_cbf} is a ZCBF
\end{lemma}
\begin{proof}
%	The main idea is that we want to show that given a proper choice of $v_r$, then physical limit on robot's speed can be respected and a value of $u$ that satisfies \eqref{eqn:tracking_constraint} can be found. 
	We start by describing $\dot{x}_r$ on its way back to the charging station. Since $\tfrac{dL}{dt} = -\left|\tfrac{dL}{ds}\right| \eta$ as discussed in lemma~\ref{lemma:base}, if we consider $\frac{dL}{dt} = -v_r$ (from lemma \ref{lemma:2}) then we can say that the value of $\eta$ needed to achieve this will be 
	\begin{equation}
	\eta_r = \frac{v_r}{\left|\tfrac{dL}{ds}\right|}
	\end{equation}
	and from \eqref{eqn:ref_pt_speed} the velocity of the reference point $x_r$ is
	\begin{equation}
	\dot{x}_r = P_{c}^{T}B^TT^{\prime}(s)\frac{v_r}{\left|\tfrac{dL}{ds}\right|}
	\end{equation} 
	and considering that $||x-x_r||^2=(x-x_r)^T(x-x_r)$ then we can multiply both sides of \eqref{eqn:tracking_constraint} by $||x-x_r||^2$ and then it can be expressed as
	\begin{equation}
	\begin{split}
	&u - \dot{x}_r \leq \gamma_dh_d\tfrac{x-x_r}{||x-x_r||}\\&u\leq P_{c}^{T}B^TT^{\prime}(s)\frac{v_r}{\left|\tfrac{dL}{ds}\right|} + \gamma_dh_d\tfrac{x-x_r}{||x-x_r||}
	\end{split}
	\label{eqn:tracking_inequality}
	\end{equation}
	provided we start in the safe set (i.e. $h_d > 0$) then the maximum value of $h_d$ inside this safe set is $h_d = \epsilon$, and the absolute value of the upper bound above can be modified so that it complies with the maximum limit on $u$, which can be expressed as
	\begin{equation}
	||u||\leq\left|||P_{c}^{T}B^TT^{\prime}(s)||\frac{v_r}{\left|\tfrac{dL}{ds}\right|} \right|+ \gamma_d\epsilon \leq ||u_{\max}||
	\label{eqn:speed_ineq}
	\end{equation}
	from \eqref{eqn:len_bez} we can differentiate $L$ with respect to $s$ using Leibniz rule to give
%	\begin{equation*}
%	\frac{dL}{ds} = f(s,\tau)\frac{d}{ds}1 - f(s,\tau)\frac{ds}{ds}+\int_{s}^{1}\frac{\partial}{\partial s}f(s,\tau)d\tau
%	\end{equation*}
	\begin{equation*}
	\frac{dL}{ds} = f(1)\frac{d}{ds}1 - f(s)\frac{ds}{ds}+\int_{s}^{1}\frac{\partial}{\partial s}f(\tau)d\tau
	\end{equation*}
	where $f(\tau) = \sqrt{\tfrac{dp_x}{d\tau}^2+\tfrac{dp_y}{d\tau}^2}=||P_{c}^{T}B^TT^{\prime}(\tau)||$ which in turn gives
	\begin{equation}
	\frac{dL}{ds} = -||P_{c}^{T}B^TT^{\prime}(s)||
	\end{equation} 
	which means that the rate of decrease in length along the path is equal to the speed with which the reference point moves along the path. Consequently \eqref{eqn:speed_ineq} becomes
	\begin{equation}
	||u||\leq v_r + \gamma_d\epsilon\leq||u_{\max}||
	\end{equation}
	then choosing a value of $v_r$ and $\gamma_d$ that satisfies the inequality above ensures \eqref{eqn:tracking_inequality} is satisfied while $||u||\leq||u_{\max}||$, i.e. choosing slower return velocity along the Bezier path makes it easier for the robot to track the reference point $x_r$ back to charging station.
	
	Since there exists a control action $u$ that satisfies \eqref{eqn:tracking_inequality}, then \eqref{eqn:tracking_cbf} is a ZCBF. 
	
%	In other words, if we choose that the reference point moves slowly along the Bezier path, then it would be easier for the robot to follow the reference point given its physical limits on speed. 
\end{proof}

One concern about the ability of the robot to go back to the charging station using \eqref{eqn:energy_suff_cbf} is the approximation error of the Bezier path length \eqref{eqn:bez_len}, since we are using Gauss quadrature to estimate the length numerically. Supposing that the true length is $\tilde{L} >0$ such that $L  = \tilde{L}\pm \epsilon$ where $\epsilon >0$ is a bounded error value, and that we consider the more critical case when $L = \tilde{L} - \epsilon$ (i.e. the length used in \eqref{eqn:energy_suff_cbf} underestimates the actual length), then substituting in \eqref{eqn:energy_suff_cbf} gives
\begin{equation*}
h_e = V - V_{\min} - \frac{k_e}{v_r}(\tilde{L}-\epsilon-\delta)
\end{equation*}
Since $V\geq V_{\min}$ outside of the charging station (by virtue of \eqref{eqn:energy_suff_cbf} being a CBF), then for $h_e$ to be equal to zero implies that $V=V_{\min}$ and $\tilde{L} = \delta + \epsilon$, i.e. at $h_e = 0$ the robot is still outside the charging station when it thinks it is on the boundary of the charging region. As a remedy, we define a modified threshold $\delta_m$ such that 
\begin{equation}
\delta_m = \delta - \epsilon
\label{eqn:modified_delta}
\end{equation} 
then using $\delta_m$ in \eqref{eqn:energy_suff_cbf} gives
\begin{equation}
h_e = V - V_{\min} - \frac{k_e}{v_r}(L-\delta_m)
\end{equation}
and by substituting $\tilde{L} = L - \epsilon$ then at $h_e = 0$ we see that $\tilde{L} = \delta_m+\epsilon = \delta$. From this we conclude that by using $\delta_m$ in \eqref{eqn:energy_suff_cbf} the robot will be inside of the charging region at $h_e = 0$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> static2.tex <==
To introduce our approach for achieving energy sufficiency, we consider a case in which a robot is static and the matrix of waypoints $\mathcal{W}$ defining the path  does not change. 
\subsection{Bezier curve construction}
We construct a cubic Bezier spline that consists of $n_w-1$ segments and passes through all waypoints as well as the robot's current position, i.e. passing through an augmented set of waypoints $\bar{\mathcal{W}} = \begin{bmatrix}
x^T&\mathcal{W}^T
\end{bmatrix} ^T \in \mathbb{R}^{(n_w+1)\times 2}$. Each one of these segments has a set of control points $\mathcal{S}_i = \begin{bmatrix}
\bar{w}_i^T& a_i^T& b_i^T& \bar{w}_{i+1^T}
\end{bmatrix}^T \in\mathbb{R}^{4\times 2}$ for $i=0,1,\dots,n_w-1$. We aim to calculate the points $a_i$ and $b_i$, which are $2n_w$ unknowns, such that $G^1$ and $G^2$ continuity is achieved at all internal waypoints $\bar{w}_i, i=1,\dots,n_w-1$, which provides a set of shape parameters to control the tightness of the interpolation. These conditions provide $2(n_w-1)$ equations. The conditions for $G^1$ and $G^2$ continuity are expressed with the following $2(n_w-1)$ equations
\begin{equation}
\begin{split}
&b_{i-1} = (1+\frac{1}{\beta_1})\bar{w}_i - \frac{a_i}{\beta_1}
\\
&b_i = \bar{w}_i + (\bar{w}_i - b_{i-1})(2\beta_1+\beta_1^2+\tfrac{\beta_2}{2}) + (a_{i-1}-b_{i-1})\beta_1^2
\end{split}
\label{eqn:cont_cond}
\end{equation}
where $\beta_1 >0$ and $\beta_2>0$ are two shape parameters. We enforce $p^{\prime\prime}_0(0)=p^{\prime\prime}_{n_w-1}(1)=0$ (i.e. free end assumption~\cite{wolberg2002energy}) to add two additional equations to the system
\begin{equation}
\begin{split}
b_0 &= 2a_0-\bar{w}_0\\
b_{n_w-1} &= \frac{\bar{w}_{n_w}+a_{n_w-1}}{2}
\end{split}
\label{eqn:term_cond}
\end{equation} 
to eventually have $2n_w$ equations and unknowns. We can express the system as two sets of $n_w$ equations to calculate $a_i$ and $b_i$. We substitute the first equation in \eqref{eqn:cont_cond} into the second, as well as \eqref{eqn:cont_cond} into \eqref{eqn:term_cond} and the result can be expressed in the following matrix form
\begin{equation}
\begin{split}
\mathcal{A} = \Psi^{-1} W\\
\end{split}
\label{eqn:a_coeff}
\end{equation}
where 
\begin{equation}
 \scalemath{0.7}{
\Psi =
\begin{bmatrix}
2 & \tfrac{1}{\beta_1}&0&0&\dots&0&0&0&0\\
\beta_1^2&\beta_1+\tfrac{\Gamma}{\beta_1}&\tfrac{1}{\beta_1}&0&\dots&0&0&0&0\\
0&\beta_1^2&\beta_1+\tfrac{\Gamma}{\beta_1}&\tfrac{1}{\beta_1}&\dots&0&0&0&0\\
\vdots&\vdots&\vdots&\vdots&\ddots&\vdots&\vdots&\vdots&\vdots\\0&0&0&0&\dots&\beta_1^2&\beta_1+\tfrac{\Gamma}{\beta_1}&\tfrac{1}{\beta_1}&0\\
0&0&0&0&\dots&0&\beta_1^2&\beta_1+\tfrac{\Gamma}{\beta_1}&\tfrac{1}{\beta_1}\\
0&0&0&0&\dots&0&0&\beta_1^2&\beta_1+\tfrac{\Gamma}{\beta_1}-\tfrac{1}{2}
\end{bmatrix}	}
\end{equation}
\begin{equation}
W =
\begin{bmatrix}
(1+\tfrac{1}{\beta_1})\bar{w}_1+\bar{w}_0\\(\tfrac{\Gamma}{\beta_1}+\beta_1^2+\beta_1-1)\bar{w}_1+(1+\tfrac{1}{\beta_1})\bar{w}_2\\(\tfrac{\Gamma}{\beta_1}+\beta_1^2+\beta_1-1)\bar{w}_2+(1+\tfrac{1}{\beta_1})\bar{w}_3\\\vdots\\(\tfrac{\Gamma}{\beta_1}+\beta_1^2+\beta_1-1)\bar{w}_{n_w-3}+(1+\tfrac{1}{\beta_1})\bar{w}_{n_w-2}\\(\tfrac{\Gamma}{\beta_1}+\beta_1^2+\beta_1-1)\bar{w}_{n_w-2}+(1+\tfrac{1}{\beta_1})\bar{w}_{n_w-1}\\(\tfrac{\Gamma}{\beta_1}+\beta_1^2+\beta_1-1)\bar{w}_{n_w-1}+\bar{w}_{n_w}/2
\end{bmatrix}
\end{equation}
\begin{equation}
\mathcal{B} = \begin{bmatrix}
(1+\tfrac{1}{\beta_1})\bar{w}_1-\tfrac{1}{\beta_1}a_1\\(1+\tfrac{1}{\beta_1})\bar{w}_2-\tfrac{1}{\beta_1}a_2\\\vdots\\ (1+\tfrac{1}{\beta_1})\bar{w}_{n_w-1}-\tfrac{1}{\beta_1}a_{n_w-1}\\\frac{\bar{w}_{n_w}+a_{n_w-1}}{2}
\end{bmatrix}
\label{eqn:b_coeff}
\end{equation}
where $\Gamma = 2\beta_1+\beta_1^2+\tfrac{\beta_2}{2}$, $\mathcal{A}\in\mathbb{R}^{n_w\times 2}$ and $\mathcal{B}\in\mathbb{R}^{n_w\times 2}$ are the matrices containing elements of $a_i$ and $b_i$. The control points of each segment $i$ are $\mathcal{S}_i = \begin{bmatrix}
\bar{w}_i^T& a_i^T& b_i^T& \bar{w}_{i+1^T}
\end{bmatrix}^T$ , for $ i=0,\dots,n_w-1$. 

We can merge the Bezier segments obtained thus far as described by \eqref{eqn:Rn} to obtain a unified set of control points $R_n$ that follows the Bezier segments, each with the control points $\mathcal{S}_i$. 
For that $P_{n_k}^k = \mathcal{S}_k$ in \eqref{eqn:Rf}, $\scriptsize\begin{bmatrix}
\left. P_1^0\right.^T&\left. P^1_1\right. ^T&\left.P^1_2\right.^T
\end{bmatrix}^T = \begin{bmatrix}
\bar{w}_0^T&a_0^T&b_0^T
\end{bmatrix}^T$ and $\scriptsize\begin{bmatrix}
\left.P^{K}\right._{n_K-2}^T&\left.P^{K}\right._{n_K-1}^T&\left.P^{K}\right._{n_K}^T
\end{bmatrix}^T=\begin{bmatrix}
b_{n_w-1}^T&a_{n_w-1}^T&\bar{w}_{n_w}^T
\end{bmatrix}^T$ in \eqref{eqn:Rc}. Figure \ref{fig:loose_tight} shows the effect of varying the values of $\beta_1$ and $\beta_2$ in the relations above.
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.48\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sharp_interpolation_results/loose.eps}
		\caption{$\beta_1 = 1, \beta_2 = 1$}
		\label{fig:loose}
	\end{subfigure}
	\hfil
	\begin{subfigure}[b]{0.48\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/sharp_interpolation_results/tight.eps}
		\caption{$\beta_1 = 1, \beta_2 = 40$}
		\label{fig:tight}
	\end{subfigure}
	\caption{Interplation of a set of waypoints (red dots) in a more relaxed manner in \ref{fig:loose} and a tighter manner in \ref{fig:tight}.}
	\label{fig:loose_tight}
\end{figure}
\subsection{Energy sufficiency over Bezier paths}
After representing the path between the robot and the charging station in the way laid out in previous section (such that the robot's position is at $\bar{w}_{0}$ and the station's position is at $\bar{w}_{n_w-1}$
%,corresponding to Bezier parameter values of $s=0$ and $s=1$ respectively
), we herein describe the CBF based framework we adopt to enable the robot to achieve energy sufficiency while moving along the Bezier path described by control points $R$. 

We consider the case in which the robot lies at the beginning of the aforementioned path and moves along this path back to the station (on the other end of the path), while the path is not changing, i.e. $\frac{dR}{dt}=0$ meaning the control points of the path are non-changing.

We start by defining a reference point along the path described as 
\begin{equation}
x_r(s) = \left(T^T(s)BR_n\right)^T = R_{n}^TB^TT(s)
\label{eqn:ref_pt}
\end{equation} 
with a parameter $s\in[0,1]$, and $R_n$ described by \eqref{eqn:Rn}. We note that the new Bezier path obtained thus far has the robot's position at $s=0$ and the station's position at $s=1$. We control the value of $s$ in a way that makes the reference point approach the end of the path in a manner that ensures energy sufficiency along the path, i.e. $V\geq V_{\min}$. For that we introduce the following dynamics for $s$
\begin{equation}
\dot{s} = \eta
\end{equation}
we then use this as a part of a constraint that drives the reference point to the end of the path, while applying another constraint that makes the robot follow the reference point.
The candidate CBF we are using for energy sufficiency is 
\begin{equation}
h_e = V - V_{m} e^{\tfrac{k_e}{v_r}(L(s) - \delta)}
\label{eqn:energy_suff_cbf}
\end{equation}
where $v_r$ is the desired velocity with which the robot moves along the path, $\delta$ is the distance of the boundary of charging region away from its center, noting that the center of the charging region is on the Bezier path at $s = 1$, and $L$ is the distance along the Bezier path from the robot's position till its end and is defined in \eqref{eqn:bez_len}.
The constraint $\dot{h}_e\geq -\alpha(h_e)$ associated with this candidate CBF is 
\begin{equation}
\begin{split}
&-k_eV-\frac{k_e}{v_r}V_{m} e^{\tfrac{k_e}{v_r}(L(s) - \delta)}\frac{dL}{dt} \geq -\gamma_e h_e\\\Rightarrow&-k_eV-\frac{k_e}{v_r}(V-h_e)\frac{dL}{dt} \geq -\gamma_e h_e
\end{split}
\label{eqn:suff_constraint}
\end{equation}
where 
\begin{equation}
\begin{split}
\frac{dL}{dt} &= \frac{\partial L}{\partial s}\frac{ds}{dt}= \frac{\eta}{2}\left[-\sum_{i=1}^{m}c_if(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right.\\&\left.+(1-s)\sum_{i=1}^{m}c_i\tfrac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})\right]
\end{split}
\label{eqn:dL}
\end{equation}
to find $\tfrac{\partial f}{\partial s}$, we define 
\begin{equation}
\begin{split}
A_i &= T^{\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})BR_n\\
A_{i}^{\prime} &=\tfrac{1-\tau_i}{2} T^{\prime\prime}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2})BR_n
\end{split}
\label{eqn:A}
\end{equation}
with $T^{\prime}(s)$ defined in \eqref{eqn:t_prime}, and 
\begin{equation}
\frac{\partial f}{\partial s}(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = \tfrac{1}{||A_i||}A_iA_i^{\prime^T}
\label{eqn:pf_ps}
\end{equation}
noting that $A_i\in\mathbb{R}^{1\times 2}$ and that $f(\tfrac{1-s}{2}\tau_i+\tfrac{1+s}{2}) = ||A_i||$. Since the change in $s$ is what changes $x_r(s)$ along the path, we introduce a constraint that lower bounds $s$ with the following candidate CBF
\begin{equation}
h_b = s
\label{eqn:lower_bound}
\end{equation}
with the associated constraint
\begin{equation}
\eta \geq -\gamma_bh_b
\label{eqn:lower_bound_constraint}
\end{equation}
We compliment \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} with another candidate CBF that aims at making the robot follow $x_r$ as it changes, and is defined as follows
\begin{equation}
h_d = \epsilon - ||x-x_r||
\label{eqn:tracking_cbf}
\end{equation} 
with $0<\epsilon< \delta$. The constraint associated with this candidate CBF is 
\begin{equation}
-\tfrac{(x-x_r)^T}{||x-x_r||}(u-\dot{x}_r)\geq -\gamma_d h_d
\label{eqn:tracking_constraint}
\end{equation}
where 
\begin{equation}
\dot{x}_r = R_n^{T}B^TT^{\prime}(s)\eta
\label{eqn:ref_pt_speed}
\end{equation}

In the following lemmas we show that the proposed CBFs thus far will lead the robot to arrive back to the charging station with $V\geq V_{\min}$. 


\begin{lemma}
	\label{lemma:base}
	For a robot with dynamics described in \eqref{eqn:robot_dynamics}, the control barrier functions defined in \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} are zeroing control barrier functions (ZCBF). Moreover, provided that $L(s)>\delta$, then $V=V_{m}$ only at  $L(s) = \delta$. 
%	Moreover, satisfying \eqref{eqn:suff_constraint} leads $x_r$ to move along the path with speed equal to $v_r$.
\end{lemma}
\begin{proof}
	Since $\eta\in\mathbb{R}$, then there exists a value of $\eta$ that satisfies both \eqref{eqn:suff_constraint} and \eqref{eqn:lower_bound_constraint} separately. We just need to show that both constraints are not contradicting. The inequality \eqref{eqn:suff_constraint} can be rewritten as 
	\begin{equation}
	\frac{dL}{ds}\frac{ds}{dt}=\frac{dL}{ds} \eta\leq \tfrac{v_r\gamma_e}{k_e}\tfrac{h_e}{V-h_e}-v_r\tfrac{V}{V-h_e}
	\end{equation} 
	but we note that $\tfrac{dL}{ds} < 0$ by definition (i.e. as we go along the path, the remaining path length decreases), thus the last inequality can be rewritten as 
	\begin{equation}
	\begin{split}
	&-\left|\frac{dL}{ds}\right|\eta\leq \tfrac{v_r\gamma_e}{k_e}\tfrac{h_e}{V-h_e}-v_r\tfrac{V}{V-h_e}\\& \Rightarrow \eta\geq-\frac{1}{\left|\frac{dL}{ds}\right|} \left(\tfrac{v_r\gamma_e}{k_e}\tfrac{h_e}{V-h_e}-v_r\tfrac{V}{V-h_e}\right)
	\end{split}
	\label{eqn:modified_he_constraint}
	\end{equation}
	therefore there is always a value of $\eta$ that satisfies \eqref{eqn:lower_bound_constraint} and \eqref{eqn:modified_he_constraint} simultaneously, thus both \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound} are both ZCBF.
	Now suppose $V=V_{\min}$, then \eqref{eqn:energy_suff_cbf} will be
	\begin{equation}
	h_e(t) =  V_{m}\left(1-e^{\tfrac{k_e}{v_r}(L(s)-\delta)}\right)\geq 0
	\label{eqn:bound_cond}
	\end{equation}
	and since $h_e\geq 0$ by virtue of being a ZCBF and since $L(s) \geq \delta$ then \eqref{eqn:bound_cond} holds only if $L(s_a) = \delta$. This means that a control input $\eta$ that satisfies \eqref{eqn:suff_constraint} leads the reference point $x_r$ in \eqref{eqn:ref_pt} to approach the boundary of charging region such that $L(s) \to \delta$.
\end{proof}

Based on the previous result, the constraint \eqref{eqn:suff_constraint} will lead the reference point $x_r$ to move along the Bezier path with a constant speed, as discussed in the next lemma
\begin{lemma}
	\label{lemma:2}
	For a robot with dynamics \eqref{eqn:robot_dynamics} and applying the constraints \eqref{eqn:suff_constraint} and \eqref{eqn:lower_bound}, the reference point $x_r$ along the Bezier path  moves back to the charging station such that $\lim\limits_{t\to\infty}\tfrac{dL}{dt} = -v_r$.
\end{lemma}
\begin{proof}
	Since the equality portion of  \eqref{eqn:suff_constraint} is activated when \eqref{eqn:suff_constraint} is violated by $u_{nom}$, we can consider the equality portion of \eqref{eqn:suff_constraint} which gives 
	\begin{equation*}
	h_e(t) = h_{e_0}e^{-\gamma_e(t-t_0)}
	\label{eqn:exp_decay}
	\end{equation*}	
	 for some initial time $t_0>0$by differentiating both sides we get
	\begin{equation}
	\begin{split}
	&-k_eV-\frac{k_e}{v_r}(V-h_e)\frac{dL}{dt}= -\gamma_eh_{e_0}e^{-\gamma_e(t-t_0)}\\
	&\Rightarrow\frac{dL}{dt} = -v_r\tfrac{V}{V-h_e} +\frac{\gamma_ev_r}{k_e}h_{e_0}e^{-\gamma_e(t-t_0)}\tfrac{1}{V-h_e}
	\end{split}
	\end{equation}
	and since $h_e(t)\to 0 $ for $t\to \infty$ due to its exponential decay, the result of $\lim\limits_{t\to\infty}\frac{dL}{dt}$ follows. We note that the speed of convergence to $v_r$ can be increased by increasing the value of $\gamma_e$.
\end{proof}

\begin{lemma}
	\label{lemma:speed_limit}
	Given a robot with dynamics as described in \eqref{eqn:robot_dynamics}, has a limited control effort $||u||\leq||u_{\max}||$ and adopting the CBFs in \eqref{eqn:energy_suff_cbf} and \eqref{eqn:lower_bound}, and provided that $v_r+\gamma_d\epsilon\leq||u_{\max}||$, then \eqref{eqn:tracking_cbf} is a ZCBF
\end{lemma}
\begin{proof}
	%	The main idea is that we want to show that given a proper choice of $v_r$, then physical limit on robot's speed can be respected and a value of $u$ that satisfies \eqref{eqn:tracking_constraint} can be found. 
	We start by describing $\dot{x}_r$ on its way back to the charging station. Since $\tfrac{dL}{dt} = -\left|\tfrac{dL}{ds}\right| \eta$ as discussed in lemma~\ref{lemma:base}, if we consider $\frac{dL}{dt} = -v_r$ (from lemma \ref{lemma:2}) then we can say that the value of $\eta$ needed to achieve this will be 
	\begin{equation}
	\eta_r = \frac{v_r}{\left|\tfrac{dL}{ds}\right|}
	\label{eqn:eta_r}
	\end{equation}
	and from \eqref{eqn:ref_pt_speed} the velocity of the reference point $x_r$ is
	\begin{equation}
	\dot{x}_r = R_n^{T}B^TT^{\prime}(s)\frac{v_r}{\left|\tfrac{dL}{ds}\right|}
	\end{equation} 
	and considering that $||x-x_r||^2=(x-x_r)^T(x-x_r)$ then we can multiply both sides of \eqref{eqn:tracking_constraint} by $||x-x_r||^2$ and then it can be expressed as
	\begin{equation}
	\begin{split}
	&u - \dot{x}_r \leq \gamma_dh_d\tfrac{x-x_r}{||x-x_r||}\\&u\leq R_n^{T}B^TT^{\prime}(s)\frac{v_r}{\left|\tfrac{dL}{ds}\right|} + \gamma_dh_d\tfrac{x-x_r}{||x-x_r||}
	\end{split}
	\label{eqn:tracking_inequality}
	\end{equation}
	provided the robot starts in a safe set $\mathcal{C}_d$ close to $x_r$ such that  $h_d > 0$, then the maximum value of $h_d$ inside this safe set is $h_d = \epsilon$, and the absolute value of the upper bound \eqref{eqn:tracking_inequality} can be modified so that it complies with the maximum limit on $u$, which can be expressed as
	\begin{equation}
	||u||\leq\left|||R_n^{T}B^TT^{\prime}(s)||\frac{v_r}{\left|\tfrac{dL}{ds}\right|} \right|+ \gamma_d\epsilon \leq ||u_{\max}||
	\label{eqn:speed_ineq}
	\end{equation}
	from \eqref{eqn:len_bez} we can differentiate $L$ with respect to $s$ using Leibniz rule to give
	%	\begin{equation*}
	%	\frac{dL}{ds} = f(s,\tau)\frac{d}{ds}1 - f(s,\tau)\frac{ds}{ds}+\int_{s}^{1}\frac{\partial}{\partial s}f(s,\tau)d\tau
	%	\end{equation*}
	\begin{equation*}
	\frac{dL}{ds} = f(1)\frac{d}{ds}1 - f(s)\frac{ds}{ds}+\int_{s}^{1}\frac{\partial}{\partial s}f(\tau)d\tau
	\end{equation*}
	where $f(\tau) = \sqrt{\tfrac{dp_x}{d\tau}^2+\tfrac{dp_y}{d\tau}^2}=||R_{n}^{T}B^TT^{\prime}(\tau)||$ which in turn gives
	\begin{equation}
	\frac{dL}{ds} = -||R_n^{T}B^TT^{\prime}(s)||
	\end{equation} 
	which means that the rate of decrease in length along the path is equal to the speed with which the reference point moves along the path. Consequently \eqref{eqn:speed_ineq} becomes
	\begin{equation}
	||u||\leq v_r + \gamma_d\epsilon\leq||u_{\max}||
	\label{eqn:abs_u_ineq}
	\end{equation}
	then choosing a value of $v_r$ and $\gamma_d$ that satisfies the inequality above ensures \eqref{eqn:tracking_inequality} is satisfied while $||u||\leq||u_{\max}||$, i.e. choosing slower return velocity along the Bezier path makes it easier for the robot to track the reference point $x_r$ back to charging station.
	
	Since there exists a control action $u$ that satisfies \eqref{eqn:tracking_inequality}, then \eqref{eqn:tracking_cbf} is a ZCBF. 
	
	%	In other words, if we choose that the reference point moves slowly along the Bezier path, then it would be easier for the robot to follow the reference point given its physical limits on speed. 
\end{proof}
Although from lemma \ref{lemma:base} we show that $V=V_m$ at $L(s) = \delta$, this is a result that concerns the reference point's position $x_r$ while the robot's actual position tracks $x_r$ through enforcing the constraint \eqref{eqn:tracking_cbf}. This implies the possibility of $x_r$ reaching the boundary while the robot's position is lagging behind. Another concern regarding the robot's ability to move along a Bezier path using \eqref{eqn:energy_suff_cbf} is the approximation error of the Bezier path length \eqref{eqn:bez_len}, since we are using Gauss quadrature integration to estimate the length numerically. 
\begin{proposition}
	\label{proposition:length_error}
	Consider a robot with dynamics \eqref{eqn:robot_dynamics} and applying the constraints pertaining to the CBFs \eqref{eqn:energy_suff_cbf}, \eqref{eqn:lower_bound} and \eqref{eqn:tracking_cbf}. Suppose that the error in length estimation due to Gauss Quadrature integration is bounded with a value $\varepsilon >0$ and that the relation between true length $\tilde{L} \geq  0$ and $L$ is 
	\begin{equation*}
	L = \tilde{L}\pm \varepsilon
	\end{equation*}
	We define a modified distance threshold $\delta_m$ as 
	\begin{equation}
	\delta_m = \delta - \varepsilon - \epsilon
	\label{eqn:delta_m}
	\end{equation}
	then using $\delta_m$ in \eqref{eqn:energy_suff_cbf} ensures that $V \nless V_m$.
\end{proposition}
\begin{proof}
	\begin{figure}[!htb]
		\centering
		\fontsize{15pt}{15pt}\selectfont% or whatever fontsize you like
		\def\svgwidth{5.333in}
		\scalebox{0.5}{\input{charging_region.pdf_tex}}
		\caption{Demonstration of a potentially curved Bezier path getting into the charging region denoted by a circle of radius $\delta$.}
		\label{fig:charging_region}
	\end{figure}
	We start by considering $\delta_m^\prime = \delta - \epsilon$. From lemma \ref{lemma:base} if $V = V_m$ at $L = \delta_m$, we consider the point $x^\prime_r$ on the path at which $L = \delta_m^\prime$. Since the length of the curved path at this point is equal to $\delta_m^\prime$, then $||x_r^\prime-x_c||<\delta_m^\prime$ as demonstrated in figure~\ref{fig:charging_region}. If we consider the robot's position to be at $x^\prime$ which is the furthest location from $x_c$ that satisfies $||x^\prime-x_r^\prime|| = \epsilon$, then
	\begin{equation}
		\begin{split}
			||x^\prime-x_c|| = ||x^\prime_r-x_c|| + \epsilon < \delta_m^\prime + \epsilon = \delta
		\end{split}
	\end{equation}
	which means by the time the reference point reaches $x_r^\prime$ at which $L = \delta_m^\prime$, the robot is ensured to be inside the charging region, i.e. $||x-x_c||<\delta$. Now we tackle the effect of the length calculation error $\varepsilon$ and we consider the more critical case when $L = \tilde{L} - \varepsilon$ (i.e. the length used in \eqref{eqn:energy_suff_cbf} underestimates the actual length), then substituting in \eqref{eqn:energy_suff_cbf} gives
	\begin{equation*}
	h_e = V - V_{m}e^ {\frac{k_e}{v_r}(\tilde{L}-\varepsilon-\delta_m^\prime)}
	\end{equation*}

If we use $\delta_m^\prime$ in \eqref{eqn:energy_suff_cbf} then $V\geq V_{\min}$ hold at $L(s) \geq \delta_m^\prime$ , then for $h_e$ to be equal to zero implies that $V=V_{\min}$ and $\tilde{L} = \delta_m^\prime + \varepsilon$, i.e. at $h_e = 0$ the robot thinks that it is at a point where $L(s) = \delta_m^\prime$ when actually it is lagging behind. As a remedy, we define a modified threshold $\delta_m$ such that 
\begin{equation}
\delta_m = \delta_m^\prime - \varepsilon
\label{eqn:modified_delta}
\end{equation} 
then using $\delta_m$ in \eqref{eqn:energy_suff_cbf} gives
\begin{equation}
h_e = V - V_{m}e^{ \frac{k_e}{v_r}(L(s)-\delta_m)}
\label{eqn:energy_suff_cbf}
\end{equation}
and by substituting $\tilde{L} = L - \varepsilon$ then at $h_e = 0$ we see that $\tilde{L} = \delta_m+\epsilon = \delta_m^\prime$. From this we conclude that by plugging $\delta_m$ in \eqref{eqn:energy_suff_cbf}, by the time $L(s)=\delta_m$ (at which case $V=V_m$ and $h_e = 0$) the robot will be indeed inside of the charging region.
\end{proof}
